Lightweight, Multi-Stage, Compiler-Assisted Application Specialization

Program debloating aims to enhance the performance and reduce the attack surface of bloated applications. Several techniques have been recently proposed to specialize programs. These approaches are either based on unsound strategies or demanding techniques, leading to unsafe results or a high overhead debloating process. In this paper, we address these limitations by applying partial-evaluation principles to generate specialized applications. Our approach relies on a simple observation that an application typically consists of configuration logic, followed by the main logic of the program. The configuration logic specifies what functionality in the main logic should be executed. LMCAS performs partial interpretation to capture a precise program state of the configuration logic based on the supplied inputs. LMCAS then applies partial-evaluation optimizations to generate a specialized program by propagating the constants in the captured partial state, eliminating unwanted code, and preserving the desired functionalities. Our evaluation of LMCAS on commonly used benchmarks and real-world applications shows that it successfully removes unwanted features while preserving the functionality and robustness of the deblated programs, runs faster than prior tools, and reduces the attack surface of specialized programs. LMCAS runs 1500x, 4.6x, and 1.2x faster than the state-of-the-art debloating tools CHISEL, RAZOR, and OCCAM, respectively; achieves 25% reduction in the binary size; reduces the attack surface of code-reuse attacks by removing 51.7% of the total gadgets and eliminating 83% of known CVE vulnerabilities

==> algorithms.tex <==
\begin{algorithm}[h!]
\caption{\lmcas Debloating Pipeline}
\label{alg:specAlg}
\DontPrintSemicolon
%\SetKwInOut{Require}{Require}
\KwIn{Program P, Supplied\_Input I}
\KwOut{Program P\textprime}
  $Constants, VisitedFunc, VisitedBB \longleftarrow \emptyset$\;
  
    \SetKwProg{Def}{def}{:}{}
    \Def{Debloat($P, I$)}{
      \tcc{\color{blue}0- Identify Neck Location}
      $L \longleftarrow FindOptimalNeckLocation ($P, I$)$\;
      $WP\longleftarrow$GenerateWholeLLVMBitCode(P)\; 
      \tcc{\color{blue}1- Run Symbolic Execution}
      $Constants, VisitedFunc, VisitedBB \longleftarrow KLEE(WP, I, L)$\;
      \tcc{\color{blue}2- Optimization Steps}
      $update(WP) \longleftarrow$ PerformOptimizationSteps(WP, Constants, 
      VisitedFunc, VisitedBB, L)\;
       \tcc{\color{blue}3- Generate specialized binary}
      $GenerateBinary(WP)$\; 
    %   $update(WP) \longleftarrow$ ConstantPropagation(WP, Constants, 
    %   VisitedFunc, VisitedBB, L)\;
    %   $update(WP) \longleftarrow$ PreNeckSimplification(WP, L)\;
    }
\end{algorithm}

\begin{algorithm}[h!]
    \caption{Differential analysis to determine global and local variables}
    \label{alg:diff}
    \DontPrintSemicolon
    %\SetKwInOut{Require}{Require}
    \KwIn{Traces (R)=$\{t_1,......,t_n\}$, args}
    \KwOut{Set of variables}
    \SetKwBlock{Begin}{Function}{end function}
    \Begin($\text{diffTraces()}$){
      Variables $\leftarrow$ \{\}\;
      Select $t_i$ $\in$ args\;
      \ForEach{var$\in t_i$}{
        \ForEach{$t \in R \textbackslash \{t_i$\}}{
    	  \uIf{value(var) has not changed}{
    	   $t_i \leftarrow$ remove($var$)\;
    	  \Else{
    	   $Variables \leftarrow$ add($var$)\;
    	  }
    	  }
        }
      }
      \Return{Variables}
    }
    \end{algorithm}
    
    
    
    \begin{algorithm}[h!]
\caption{\lmcas Multi-Stage Simplification}
\label{alg:optimization}
\DontPrintSemicolon
\KwIn{PW, Constants, VisitedFunc, VisitedBB}
\KwOut{Program P\textprime}
  $VarWorkList, FuncWorkList \longleftarrow \emptyset$\;

    \SetKwProg{Def}{def}{:}{}
    \Def{MultiStageSimplification($WP, I$)}{
      \tcc{\color{blue}3- Pre-neck Simplification Step}
        \For{$arg \in pre\_L$}{
            \If{$arg != I$}{
                $recordVarsFuncs(arg)$\;
                $removeBlock(arg)$\;
            }
        }
      \tcc{\color{blue}4- Post-neck Simplification Step}
        \For{$condition \in post\_L$}{
            \If{$condition == false$}{
                $recordVarsFuncs(condition)$\;
            } \uElseIf{$condition == true$}{
                $condition.remove()$\;
            } 
        }
      \tcc{\color{blue}5- Cleaning Step}
        \For{$func \in FuncWorkList$}{
            \If{$notInvoked(func) == true$}{
                $recordVarsFuncs(func)$\;
            }
                $remove(func)$\;
            }
        
       \For{$var \in VarWorkList$}{
            \If{$notUsed(var) == true$}{
                $remove(var)$\;
            }
        }
    }
    
    \SetKwProg{Def}{def}{:}{}
    \Def{recordVarsFuncs($location$)}{
        \For{$instr \in BasicBlock(location)$}{
            \uIf{$instr \in variable$}{
                $VarWorkList \longleftarrow instr$\;  
            } \uElseIf{$instr \in CallSite$}{
                $FuncWorkList \longleftarrow instr$\; 
            }
        }
    }
\end{algorithm}

==> approach.tex <==
\section{\lmcas Framework}
\label{sec:approach}

This section introduces \lmcas, a lightweight debloating framework that uses sound analysis techniques to generate specialized programs. 
Figure~\ref{fig:approach} illustrates the architecture of \lmcas. 
The debloating pipeline of \lmcas receives as input the %source code of program $P$, and
whole-program LLVM bitcode of program $P$, and\Omit{\twr{wording changes}}
performs the following major steps to generate a specialized program $P\textprime$ as bitcode, which is ultimately converted into a binary executable.
\Omit{\twr{Is the overall transformation bitcode-to-bitcode? source-to-bitcode? source-to-binary? bitcode-to-binary? Somewhere we used to say that neck identification was performed on the source code---I may have removed that phrase; that seems like an inessential detail: it may be how it is done in our implementation, but I would expect that, in principle, there is nothing that precludes it from being carried out on the bitcode.} \ma{If we consider that in principle, the neck can be specified on top of the bitcode, then our overall transformation is bitcode-to-bitcode. If this makes sense, I'll do the required changes}}

\begin{itemize}
    \item \textbf{Neck Identification Requirements (Section~\ref{subsec:neck}).} As mentioned in Section~\ref{subsec:challenges}, the \textit{neck} is used to partition the code into the part on which symbolic execution is applied, and the part on which a number of optimizing transformations are applied.\Omit{\twr{Reworded:}}
    In our current system, neck identification is performed manually.
    Section~\ref{subsec:neck} discusses neck identification, and formalizes the problem for which we plan to develop automatic support.
    \Omit{\vr{This seems wrong. We do not have an algorithm but only a formalization of the problem we need to solve.} \ma{ture}}
    \item \textbf{Symbolic Execution (Section~\ref{subsec:SE}).} 
    Symbolic execution executes the original application up to the neck, based on a set of supplied inputs that control which functionality should be supported by the specialized application.
    The output of the symbolic-execution phase provides (i) a set of global and stack variables and their corresponding values, and 
    \Omit{\twr{Clarify: presumably this refers to visited functions and basic blocks \emph{up to the neck},} \ma{Yes, thanks for the clarification}}
    (ii) a record of the visited functions and their basic blocks up to the neck. %The Specialization applies partial evaluation~\cite{partialEvaluation}, where a specific set of variables are frozen to fixed values.
    \item \textbf{Constant Conversion (Section~\ref{subsec:cc}).}
    This phase converts the variables and their corresponding values captured after symbolic execution (i.e., $V_s$ and $C_s$) to settings of constants at the neck.
    This phase also takes advantage of the opportunity to boost the degree of subsequent optimization steps by (i) supporting the conversion of multiple kinds of data types to constants, and (ii) performing constant-conversion in both the configuration logic and the main logic of the program.
    \item \textbf{Multi-Stage Simplification (Section~\ref{subsec:msp}).}
    This phase applies selected standard and customized LLVM passes for optimizing the program and removing unnecessary functionality.
    These optimization steps are arranged and tailored to take advantage of the contribution provided by the constant-conversion phase. 
\end{itemize}

\begin{figure}[tb]
    \centering
    % 
    \includegraphics[width=9cm, height=3cm]{images/debloating_v2.png}
    \caption{Overview of \lmcas.}
    \label{fig:approach}
\end{figure}


%All of these steps are performed on top of the LLVM bitcode~\cite{LLVM:CGO04}, except for the \textit{neck identification} step, where the analysis relies on the source code (see Figure~\ref{fig:neck}). 

%from \cite{EuroSec19}
%Challenges:: First, the code that is related to a particular configuration directive needs to be precisely identified. Second, the rest of the code must be analyzed to ensure that it does not depend on the code that will be removed if that particular directive is disabled.

%An ideal approach would take a configuration directive as input, automatically identify all associated code, and extract the subset of that code that is not needed by the rest of the program when this particular functionality is disabled. 

%Unneeded code removal can be performed at different levels of granularity, e.g., at the instruction, function, or library level

%expository purposes
%All analyses and transformations occur on LLVM bitcode

%Our lightweight specialization approach interleaves \textit{Symbolic Execution} and \textit{Partial Evaluation} in a sound way to specialize applications. We execute the original application based on a set of supplied inputs, which represent the functionality that will be supported by the specialized application. The symbolic execution provides 1) a set of global and local variables that will be turned into constants and 2) records the visited functions and their basic block. The Specialization applies partial evaluation~\cite{partialEvaluation}, where a specific set of variables are frozen to fixed values.  
%Running the residual program on the remaining input data will yield the same result as running the original program on all of its input data
%1) converts variables to constants, 2) performs constant propagation, and 3) simplifies the code. Following is a detailed discussion of each component:

%To optimize the symbolic execution, our approach interrupts the symbolic execution up to a certain point in the application. The symbolic execution also records the invoked functions and the visited basic blocks. 

%To this end, we run the symbolic execution and enable various configuration options each time. The differential analysis keeps the variables whose values have been changed among the different symbolic executions. 

\subsection{Neck Specification} \label{subsec:neck}
\input{neck}

\begin{comment}
    The neck defines a splitting point between configuration and main logic in a program $P$ as illustrated in Figure~\ref{fig:neck}. Identifying this location accurately is of paramount importance to optimize and conduct sound analysis. The neck has two major functionalities: (1) terminating the execution of the symbolic execution after reaching the neck. Hence, our neck identification algorithm should be able in an airtight manner to distilling the variables influenced by the supplied inputs. 2) providing boundaries where constant propagation should be performed. All variables captured in the symbolic execution that their uses are located before the neck, they can be safely converted to constants. %But after the neck if the variable is after the neck and is modified, then we cannot convert this variable to constant.
    
    In order to automatically identify the location where the symbolic execution should be interrupted, we define the neck identification criteria as a tuple L= <I, V, C, F>, where:
    \begin{itemize}
        \item \textbf{I} is a set of supplied inputs that activate the intended functionality. These inputs can be in the form of command-line arguments. 
        \item \textbf{V} is a set of variables that will be affected by the identified inputs \textit{I} and contribute to the activated functionality. This set comprises local and global variables. 
        \item \textbf{C} is a set of constant values that correspond to the set of variables \textit{V}.
        \item \textbf{L} is the location of the neck in the original application and based on it we identify the relevant variables \textit{V}.  
        \item \textbf{F} is a functionality that will be supported by the specialized application based on the given set of inputs \textit{I}. This functionality should be provided after running the specialized application. 
    \end{itemize}

    To verify if the selected neck location \textit{(L)} is the optimal, the functionality \textit{(F)} should be satisfied after generating the specialized app P\textprime. Otherwise, we keep iterating new nick locations until the functionality \textit{(F)} is satisfied. This process can be guided by relying on heuristic analysis. For example, GNU Core Utilities apply the same approach for parsing the inputs \textit{(I)}.
\end{comment}


\subsection{Symbolic Execution (SE)} \label{subsec:SE}
    The symbolic-execution phase is a supporting phase whose goal is to identify---at the neck---the set of variables (and their values) that contribute to the desired functionality.
    Symbolic execution is performed only up to the neck;
    all functions and basic blocks visited during symbolic execution are recorded.
    After symbolic execution terminates, the current symbolic state is saved, and the values of all variables are extracted.
    Different types of variables are extracted, including base types (e.g., \texttt{int}, \texttt{char}) and constructed/compound types (e.g., \texttt{enum}, pointer, array, and \texttt{struct}). 
    
    \Omit{\twr{Omit starting with
    ``Our approach supports capturing these various types of data types to perform a sound analysis.''  I think it is something you've written to defend/distinguish your work w.r.t. CHISEL, OCCAM, and TRIMMER, but it is only intrusive in the presentation of \emph{your} work.} \ma{I agree}}
    
    \Omit{\twr{Does the following sentence capture what you intended to say?} \ma{ Yes}}
    Consider a network-monitoring tool, such as \texttt{tcpdump}, that supports multiple network interfaces, and takes as input a parameter that specifies which network interface to use.
    A specialization scenario might require monitoring a specific interface (e.g., Ethernet) and capturing a specific number of packets: for \texttt{tcpdump}, the command would be ``\texttt{tcpdump -i ens160 -c 100}'' (see the inputs listed in Table~\ref{tab:largeApps}, Section~\ref{sec:evaluation}).
    The first argument identifies the Ethernet interface $\texttt{ens160}$, while the second argument specifies that the number of packets to be captured is $100$.
    The former argument is a string (treated as an array of characters in C) and the latter is an \texttt{int}.
    \Omit{\twr{Omit the following sentence: I don't think it adds anything:}}
    %(These argument types are different from the ones illustrated in the motivating example (\texttt{-lc}), which are characters.)
    
    Returning to the example from \S\ref{sec:motivation} (Listing~\ref{wc}), Figure~\ref{fig:neck} illustrates the location of the neck.
    Suppose that the desired functionality is to count the number of lines (i.e., \texttt{wc -l}).
    Table~\ref{tab:vars} shows a subset of the variables and their corresponding values that will be captured and stored in \lmcas's database after symbolic execution finishes.
    %However, the list of captured variables is longer (i.e., other environment variables), but Table~\ref{tab:vars} lists the relevant variables. 
    
    \begin{table}[!htb]
    \centering
    \caption{The set of captured variables $V_s$ and the corresponding values obtained after symbolic execution.}
    \begin{tabular}{lllc}
        \hline
        Variable & Type & Scope & Value \\ \hline
        \texttt{total_lines} & \multirow{2}{*}{\texttt{int}} & \multirow{2}{*}{Global} & 0 \\
        \texttt{total_chars} &                   &                   & 0 \\ \hline
        \texttt{flag->count_lines} & \texttt{int} & \multirow{2}{*}{Local} & 1 \\
        \texttt{flag->count_chars} & \texttt{char} &                   & 0 \\ \hline
    \end{tabular}
    \label{tab:vars}
    \end{table}
    

    %The set of variables \textit{(V)} may include a myriad of variables. Since not all variables in \textit{(V)} contribute to the required functionality to be enabled in the specialized application. Therefore, this step removes all variables in \textit{V} that are irrelevant. Removing irrelevant variables: 1) reduces the overhead of the specialization process and 2) supports generating accurate specialized applications. We apply two techniques to identify relevant variables: \textit{visited locations} and \textit{differential analysis}. 
    
    %Algorithm~\ref{alg:diff} describes our differential analysis approach. The user provides a pair of executions to denote different functionalities. One execution containing the trace of the intended functionality enabled by the inputs. The other containing a trace of another functionality that is not related to the enabled one. The algorithm prunes variables that are common in both traces and hence not required to perform the specialization. 
    
    %The algorithm determines the specific set of global and local variables that will be fed to the LLVM pass where the specialized application will be generated.

\subsection{Constant Conversion (CC)} \label{subsec:cc}

\Omit{\twr{I don't understand why you have to do constant conversion in the main logic.
After constant conversion in the pre-neck, why don't all the post-neck simplifications fall out for free via the constant propagation and \texttt{simplifycfg}? \ma{standard constant propagation LLVM pass perform mainly constant folding see (https://releases.llvm.org/6.0.0/docs/Passes.html\#constprop-simple-constant-propagation) i.e., x = 3 + 4 becomes x = 7 (I tested x1= 1, x2= 2, x= x1+x2, but the constprop pass hasn't done constant propagation for x1 and x2 by making x=20), are limited to global variables, and don't handle data types required for our analysis. I also tried the other LLVM pass ipconstprop on the previous example but doesn't propagate constant in the previous example. Furthermore, constant propagation passes don't account for aliasing, therefore we need to perform the post-neck CC. \texttt{simplifycfg} does folding only for control-flow instructions for simplifying and merging BBs. I'll add this explanation at the beginning of Main-logic CC, as we discussed}}
\vr{I agree with Tom here. When you consider LLVM optimizations, you have to consider all of them together, not pick out just one and test it alone. I tested your example and LLVM handles it perfectly.}}
\Omit{\twr{Wording changes OK?}\ma{Yes, thanks}}
We perform constant conversion for variables not only before the neck but also after the neck. These conversions enable further simplifications in later steps.
Constant conversion is performed in two steps: \textit{Configuration Logic Constant-Conversion} and \textit{Main Logic Constant-Conversion}. These two steps are discussed below.

\noindent\textbf{Configuration Logic Constant-Conversion.}
This step aims to propagate constants in the configuration logic to achieve further optimizations. The constant conversion is performed upstream of the neck, thus the variables in the configuration logic are converted to constants in a backward direction based on the captured vales at the neck. 
\twr{If I were a reviewer, the following sentences would raise a red flag with me.  They sound like nonsense: are you replacing occurrences of variables in the pre-neck with their values at the neck?  That can't be right: an occurrence $vo$ of variable $v$ can only be replaced with a constant value $c$ if (i) $c$ was the only value that $vo$ took on whenever that point in the program was reached, and (ii) the replacement value is $c$.
But what if the value of $v$ at the neck is $c'$ and not $c$.  Will you replace $vo$ with $c$ or $c'$? When I read this paragraph, it leads me to think that $vo$ is replaced by $c'$, because I don't see anything that makes me think that you have captured the earlier value $c$.}
The def-use chain of global and stack variables is utilized to replace all occurrences of the variables with their corresponding constant values in the program code before the neck. 
\twr{The following sentence is problematic.
Yes, some of the statements will become dead, but not all of them do, and you still have to perform a sound transformation of the pre-neck.}
Because some of the program statements will become dead after constant-conversion, the replacement is performed for all occurrences of the set of variables obtained after symbolic execution.
Algorithm~\ref{alg:cc} describes the transformations that are performed during this step. The algorithm receives as input the bitcode of the whole program $P$ generated using WLLVM\footnote{https://github.com/SRI-CSL/whole-program-llvm}, as well as a dictionary (similar to Table~\ref{tab:vars}) that maps the set of variables in $V_s$ captured after symbolic execution and their constant values $C_s$. The set $V_s$ involves global and stack variables (base-type, struct, and pointer variables). 

Algorithm~\ref{alg:cc} iterates over the IR instructions to identify
the locations where the variables are accessed, which is indicated by load instructions at Line~\ref{alg:l:fndLoadInst}. Then, we replace the loaded value with the corresponding constant value. 
%load instructions (\texttt{LoadInstr}) and check their operands. Load instructions are where the conversion is directly performed.
%and Get Element Pointer instructions (\texttt{GEPInstr}).
%Load instructions are where the conversion is directly performed.
This approach works for global variables (Lines~\ref{alg:l:globals-b}-\ref{alg:l:globals-e}) and stack variables with base types (Lines~\ref{alg:l:base-b}-\ref{alg:l:base-e}). %, except the operand check type. The operand should belong to the set global variables (Line 5) to convert global variables to constants, while the operand should be an Allocation Instruction (\texttt{AllocInstr}) (Line 11). 
But for pointers to base variables, Algorithm~\ref{alg:cc} identifies locations
where the pointer is modifying the base variable by looking for store
instructions whose destination operand belongs to the list of pointer variables to base type at Line~\ref{alg:l:PtrBaseVars}.\Omit{\vr{grammar seems off} \ma{where?}}\Omit{\vr{see if
the rewording of the previous sentence is ok. You have not defined what PtrBaseVars is.}\ma{Fixed the PtrBaseVars}} We then replace the source operand of the store operation to use the constant value corresponding to the actual base variable pointed to by the pointer (Lines \ref{alg:l:PtrToBase-replc1}-\ref{alg:l:PtrToBase-replc2}).
%all occurrences of global variables\texttt{total\_lines} and \texttt{total\_chars} before the neck are replaced with their corresponding constant values in Table~\ref{tab:vars}.
% store instructions (\texttt{StoreInstr}) that maintain \texttt{AllocInstr} operand belongs to the list PtrBaseVars. The type of these \texttt{AllocInstr} operands is a pointer, unlike the \texttt{AllocInstr} operands of the base type variables. 
\Omit{\vr{How do you handle pointer to pointer} \ma{both pointers point to the same memory location. Therefore, the constant values obtained from KLEE are based on the last modification and thus we don't need to apply alias/pointer analysis}\vr{This is important and is still not addressed. You would need a more general solution using a points-to analysis like you do for main logic.}}

Stack variables that are Structs and pointers to Structs are handled at Lines~\ref{alg:l:strctPtrToStrct-b}-\ref{alg:l:strctPtrToStrct-e}, we first need to identify the memory address that is pointed to by these variables using \Omit{\twr{What exactly is \texttt{GEPInstr}?}}
\texttt{GEPInstr} at Line~\ref{alg:l:strctPtrToStrct-b}.
%This dereferencing step 
\texttt{GEPInstr} facilitates tracing back to finding the corresponding struct and pointer-to-struct variables at Line~\ref{alg:l:strctPtrToStrct-traceBack}.
The algorithm then at Line~\ref{alg:l:strctPtrToStrct-findStor} iterates the occurrences of the \texttt{GEPInstr} by leveraging the LLVM method \texttt{users()} to identify store operations that modify the variable. %The variable modification is identified through the presence of a store operation whose destination operand is the intended variable. 
Finally, it converts the source operand of the store operations to become constant, thus it reinforces the new constant value as described at Line~\ref{alg:l:strctPtrToStrct-e}. % which are replaced with a new \texttt{StoreInstr} that points to the required constant value. 
%The \texttt{users()} API offers an easy way to access the def-use chain~\cite{spa}. Therefore, we can get a list of all instructions that are using the intended instruction. 
%In LLVM, pointer and Struct variables can be modified and accessed by Store Instruction (\texttt{StoreInstr} and \texttt{LoadInstr}) indirectly, after obtaining the actual location of the \texttt{AllocInstr}. This location is computed using the \texttt{GEPInstr} and used by \texttt{StoreInstr} and \texttt{LoadInstr}. Therefore, we trace back to find the corresponding \texttt{AllocInstr} that belongs to the local variable (based on the index that is recorded in the symbolic execution). After identifying \texttt{GEPInstr}, we check if its operand is an \texttt{AllocInstr} and the index of this \texttt{AllocInstr} is recorded in the lists $StructVars$ or $PtrVars$. We then iterates the use of the \texttt{GEPInstr} by leveraging the LLVM method \texttt{users()} to identify \texttt{StoreInstr}, which are replaced with a new \texttt{StoreInstr} that points to the required constant value. The \texttt{users()} API offering an easy way to access the def-use chain~\cite{spa}. Therefore, we can get a list of all instructions that are using the intended instruction. \Omit{\twr{Clarify: what do you mean by ``the memory address that is pointed out by these variables''.  Maybe you should tell the reader what GEPInstr does.} \ma{ I'll do}} \Omit{\ma{I added the description to the previous paragraph.}}. 
In addition to the tracing back, we also use the recorded element index in symbolic execution to identify which struct element should be converted.
For instance, in the motivating example, the struct pointed to by \texttt{flag} consists of two elements (\texttt{count\_lines} and \texttt{count\_chars}), so we maintain their indices correctly to perform an accurate constant conversion.

For string variables, Alogrithm~\ref{alg:cc} identifies the instructions that represent string variables %\texttt{AllocInstr} 
at Line~\ref{alg:l:strgVar}. It then creates an array and assigns the string to the created array, which will be converted to a global variable (Lines~\ref{alg:l:crtAry}-\ref{alg:l:crtGbl}) because LLVM treats strings as global variables. Finally, the algorithm identifies store instructions that use the string variable as its destination operand, and overrides source operand of the store instruction to use the constant string value assigned to the created global variable (Lines~\ref{alg:l:findstrStore}-\ref{alg:l:replaceStoreStr}).

According to the motivating example (see Listing~\ref{wc}), no replacement is performed for the global variables \texttt{total\_lines} and \texttt{total\_chars} before the neck, because of the absence of any occurrences. But the replacement is performed for the elements of the pointer to the struct \texttt{flag}. Therefore, the occurrences of $\texttt{flag->count\_chars}$, $\texttt{flag->count\_lines}$ at lines 13 and 14 are replaced with the their corresponding constant values listed in Table~\ref{tab:vars}.

%Finally, we use the LLVM API \texttt{ReplaceInstWithValue} to accomplish the constant conversion by performing the replacement of the \texttt{StoreInstr}. We also leverage the LLVM method \texttt{ReplaceInstWithValue} to perform the conversions at lines 7,9,13, and 15.
% Algorithm~\ref{alg:cc} describes the transformations that are performed during this phase. The algorithm receives as input the bitcode of the whole program $P$, as well as the set $V_s$ of the captured variables after symbolic execution.
\Omit{\twr{In Line 3, the iteration is over \emph{every} instruction of $P$.  However, I thought constant-conversion was only performed on the post-neck portion of $P$.  I thought some different algorithm was employed to simplify the pre-neck portion. \ma{I got your point about the iteration, I'll modify the algorithm to stop instruction iteration at the neck. For example if there is a condition located before the neck `if (x)`, and SE provided the value of x is 0, this means the condition is always false, so I need to convert x here to 0 though it's before the neck, therefore the simplifyCFG can recognize this branch will not be taken and thus simplifies it. Otherwise, simplifyCFG can't remove the branch} In any case, it does not seem sound to use the values from the neck in the pre-neck portion: the values are the result of a computation performed by the code up to the neck.}\ma{I need to do the pre-neck CC, because this will facilitate the simplification steps that will be performed subsequently.}} 

The constant conversion operates using updated and accurate values, because symbolic execution phase handles situations where a pointer indirectly updates the value of a memory location. 
% $V_s$ contains a list of global and stack variables, which consist of base-type, struct, and pointer variables. 

\Omit{The set of global variables may include a plethora of variables (not just the variables in Table~\ref{tab:vars}).
However, not all global variables in $V_s$ contribute to the functionality that the \lmcas user desires to enable in the specialized program. Therefore, the constant-conversion step at Line $2$ removes global variables in $V_s$ that are irrelevant.
Removing irrelevant variables 1) reduces the overhead of the specialization process, and 2) supports generating accurate specialized applications by avoiding side effects (i.e., \Omit{\twr{How can missing a variable cause a side effect?} \ma{crashing, run forever, wrong output}} missing a variable, or converting at a wrong location)\Omit{\twr{``resulted after the constant conversion'' is not grammatical; do you mean ``caused by constant conversion''?} \ma{ yes}}
% resulted after the constant conversion. 
caused by constant conversion
\Omit{\vr{This paragraph is very confusing to me. Do we have some examples of
variables that are irrelevant? \ma{e.g., argc} I too do not see why this should be required.
Moreover, Line 2 is a blackbox. Can you explain the algorithm for
FilterGlobalVars()? \ma{explained in the next paragraph "irrelevant global variables will be removed by comparing"}}}}

\Omit{\twr{You say ``all irrelevant variables'' whereas I would say just ``irrelevant variables.''  It is a red flag to say ``all'' because the problem of identifying irrelevant variables is undoubtedly undecidable.  Now it occurs to me that the problem statement for this phase must be ``Identify a subset of all definitely relevant variables,'' which means that you are over-approximating the set of (all) irrelevant variables.} \ma{Thanks for explaining that. I agree.}}
\Omit{\twr{Please start the paragraph by saying what the purpose of this filtering step is.
In hidden notes, you seemed to have agreed that the specification of the step is to identify a "subset of all definitely relevant variables".
You seem to be achieving that by removing an overapproximation of irrelevant variables.
}}%The set of global variables may include a plethora of variables (not just the variables in Table~\ref{tab:vars}). Irrelevant variables are filtered out by identifying the intersection with the list of global variables obtained through the LLVM pass. 
%leveraging information captured after symbolic execution.
%The names of global variables and indices of stack variables in each function are recorded as well.
\Omit{
\twr{I don't understand what Line 2 does: if SE gives you a set of global variables, and LLVM gives you the set of all global variables, what are you checking for?  At best you can check that the former is contained in the latter.} \ma{yes, this is exactly what I did, check intersection between LLVM list and KLEE list of global variables}
\twr{If SE has supplied a set of \emph{global variables} in parameter \textit{GlobalVars}, you already know that they are global variables, and hence it is unnecessary to check that they are global variables w.r.t. the LLVM list.  Your implementation may perform such a check as a way to catch bugs, but there is no reason to include such a check in the pseudo-code---it is just an irrelevant detail.}\ma{Agreed, it's not a major step. I will remove it from the algorithm and from the text.}}
%Irrelevant global variables are removed (\texttt{FilterGlobalVars} at Line 2) by identifying the intersection with the list of global variables obtained through the LLVM pass.% method \texttt{getGlobalVariable()}.

% We perform the constant-conversion for variables not only before the neck but also after the neck. This conversion leads to further simplifications. The constant-conversion is performed over two steps: \textit{Configuration Logic Constant-Conversion} and \textit{Main Logic Constant-Conversion}.
% These two steps are discussed below.

\noindent\textbf{Main Logic Constant-Conversion.}
%We perform the constant-conversion for variables not only before the neck but also after the neck. This conversion will lead to further simplifications.  
\Omit{\vr{incomplete sentence.}\ma{thanks. I fixed it}}This step is applied only for the set of variables that are not modified in the main logic.\Omit{\twr{Not understanding ``by iterating the usage of the variable''.  It sounds like you are doing reachability in some kind of graph (built as part of the LLVM IR?)  Can you describe it that way?} \ma{ I added a description in the 1st place when I mentioned the API users()}}
%We identify variables with this property by iterating the usage of the variable after the neck by leveraging the def-use chain provided by LLVM.\Omit{\twr{The issue that comes to mind is ``How are you accounting for aliasing?'' For instance, how do you know that an object is not modified through a pointer?  Perhaps the answer is obvious to someone who knows LLVM, but don't assume that your reader (or co-author :) ) knows.} \ma{I'll try to address the aliasing point. I'll add this to the discussion section. But I already mentioned in the discussion section that we need to perform pointer analysis. }}
\Omit{\twr{wording changes OK -- to end of paragraph?}\ma{Yes, thanks}}We identify variables with this property using the def-use chain at each variable occurrence of interest.
The absence of a store instruction indicates that no write operation is performed on the variable;
in this case, the value of the variable is not changed after the neck, and it is safe to perform the constant-conversion. \Omit{\twr{Something is definitely incorrect here: This is the section about \emph{main-logic} constant-conversion, but Algorithm~\ref{alg:cc} is for \emph{configuration logic}}\ma{I'll fix it} \vr{looking forward to seeing the fix/}\ma{I need to revisit. I'm not quite sure how to put preneck and postneck in one algorithm}}%which is carried out according to Algorithm~\ref{alg:cc}. 
Although LLVM provides a set of standard constant propagation passes, these passes do not handle data types considered in our analysis, mainly perform constant folding, and lack of handling aliasing. Therefore, we also adapt our Algorithm~\ref{alg:cc} to address the challenges presented by aliasing~\cite{PGL-014}, as described at Lines~\ref{alg:l:alias}-\ref{alg:l:alias-e}:
constant-conversion should be performed for
a variable occurrence only if it can be shown that it is not written to after the neck, either directly or via an alias.
Generally, our analysis needs only to be worried about aliasing for a small set of variables maintained by the dictionary $Map$ (mapping of $V_s$ to $C_s$ in Algorithm~\ref{alg:cc}).
To this end, we use LLVM alias-analysis APIs to obtain the set of all variables that might write to the memory locations in which we are interested. \Omit{\vr{Can we add a bit more detail? As a reviewer, I will be interested in words like ``interprocedural'' and ``may-alias.''}\ma{I explained mayAlias, not quite sure where are you referring to by interprocedural}}\Omit{\ma{I don't want to put low-level details, but in case you've any concerns, LLVM provides an API to perform AliasAnalysis, so my implementation leverage these APIs to provide me the set of aliases (mayAlias not mustAlias, over-approximate, but to avoid wrong constant conversion) of a certain memory location, then I check if none of them is modified after the neck to proceed with the CC. Just to be clear, I haven't implemented the AliasAnalysis, it's provided by LLVM}}%(1) two or more pointers point to the same memory address and (2) a pointer to a variable. 
Finally, the constant conversion is performed after all these variables are examined to verify they do not make any modification after the neck.
%The absence of a store instruction indicates no write operation will be performed on the variable, thus the value of the variable is not changed after the neck, and it is safe to perform the constant-conversion. 

\Omit{\vr{slightly reworded this para}\ma{thanks}}
In the motivating example (see Listing~\ref{wc}), the global variables \texttt{total\_lines} and \texttt{total\_chars} are not converted to constants because their values are modified after the neck at Lines 17 and 18. However, the struct elements $\texttt{flag->count\_chars}$, $\texttt{flag->count\_lines}$ used in the conditional statements at Lines 17-20 are replaced with the their corresponding constant values listed in Table~\ref{tab:vars}. This makes the conditions at Lines 17 and 19 always false, but the conditions at Lines 18 and 20 are always true. These post-neck constant-conversions facilitate the simplifications performed in the next phase Multi-Stage Simplification. 

%The symbolic execution captures the updated and recent \vr{what does updated and recent even mean in this context?} \ma{means if we have such variables int i = 2; int *p; p = \&i; *p = 10; then the value of i is 10 not 2, this is what I meant by updated/recent} \ma{plz help to reword} constant values obtained from the memory. This implies the constant conversion before the neck will be consistent and based on accurate values, which overcomes the challenge imposed by aliasing~\cite{PGL-014}. While the post-neck conversion is performed if none of the aliases is writing to the memory. To this end, we capture two perceptions about variables involved in the aliasing (1) two or more pointers point to the same memory address and (2) a pointer to a base variable. For the first perception, it is identified when we capture constant values of pointer variables after the symbolic execution, we also capture if they point to the same memory address while processing the captured KLEE state. While for the second perception, we rely on modeling the operation of assigning a variable to a pointer in the configuration logic. Specifically, the presence of \texttt{StoreInstr} that writes the variable address of an \texttt{AllocInstr} maintained by the pointer variable. The goal of these perceptions is not to substitute alias analysis, rather it provides us a lightweight analysis to decide the post-neck constant-conversion, %, which will only be performed if the pointer changes the values by leveraging \texttt{StoreInstr}, then the constant-conversion will not be executed. 

% \ma{the main issue here, if the pointer is modifying the object after the neck, but we convert the variable itself after the neck because no write operation on the variable itself. This is wrong because the pointer is modifying the variable after the neck, this reflects there should be no post-neck conversion on the variable. This is a limitation that we have in the current work}.
\Omit{\vr{The language needs improvement, I am not able to understand much of the
stuff here. Do we have a pointer analysis or not? \ma{No, that's why I didn't mention that. I basically, was benefiting from def-use chain API provided by LLVM. A single storeinstr after the neck indicates the variable's value is modified and I was doing this for all variables in case of pointer to variable} Note that we can work with a
conservative analysis that provides soundness guarantees. For example, if the
address of a variable is never taken, we can make it constant without worry. \ma{I don't get your point here "Note that we can work with a conservative analysis ... without worry", because I think what you described here is a summary of the previous paragraph.}}}

\begin{comment}
\begin{algorithm}[!htb]
% \scriptsize
\small
\caption{\lmcas Constant-Conversion}%\lmcas Constant Conversion
\label{alg:cc}
\DontPrintSemicolon
\KwIn{program P, Map <$V_s, C_s$>,%$V_s$=\{$Globals$, $BaseVars$, $PtrBaseVars$,$StringVars$, $PtrStrctVars$, $StructVars$\}, 
L=$NeckLoc$}
\KwOut{$P_{cc}$}
%   $VarWorkList, FuncWorkList \longleftarrow \emptyset$\;
    \SetKwProg{Def}{def}{:}{}
    $P_{cc} \longleftarrow P$ \;
    % \Def{ConstantConversion($P, GlobalVars, LocalVars$)}{
    %   FilterGlobalVars(GlobalVars) \;
       \Repeat{$Instr \neq L$}{
       \For{$Instr \in P_{cc}$}{
        \If{$Instr$ is $LoadInstr$}{
            \textcolor{blue}{\tcc{Handle Global Variables}}
            \If{$Instr(oprnd) \in Globals$}{
                $replaceWithConst(oprnd)$\;
                % \If{oprnd before $L$}{
                %     $replaceWithConst(oprnd)$\;
                % } 
                % \uElseIf{operand after $L$ \&\& $accessOnlyAfterNeck(oprnd)$}{
                %     $replaceWithConst(oprnd)$\;
                % }
            }
            \textcolor{blue}{\tcc{Handle Base Variables}}
        % \If{$Instr$ is $LoadInstr$}{    
            \If{$Instr(oprnd) \in AllocInstr$ $\land$ $oprnd \in BaseVars$}{
                $replaceWithConst(oprnd)$\;
                % \If{oprnd before $L$}{
                %     $replaceWithConst(oprnd)$\;
                % }
            }
        % }
        }
        \textcolor{blue}{\tcc{Handle Pointer to Base Variables}}
         \If{$Instr$ is $StoreInstr$}{    
            \If{$Instr(oprnd2) \in AllocInstr$ $\land$ $Instr(oprnd) \in PtrBaseVars$}{ \label{alg:l:PtrBaseVars}
                \If{oprnd before $L$}{
                    new $\longleftarrow$ createStoreInstr(oprnd.val)\;
                    ReplaceInstWithInst(Instr, new)\;
                }
            }
        }
        
        \textcolor{blue}{\tcc{Handle Struct \& Pointer to struct Variables}}
        \If{$Instr$ is $GEPInstr$}{
            \If{$Instr(oprnd)$ is $AllocInstr$ $\land$ $Instr(oprnd) \in \{StructVars, PtrStrctVars\}$}{
                \For{$us \in use(Instr)$}{
                    \If{$us$ is $StoreIntr$}{
                        new $\longleftarrow$ createStoreInstr(oprnd.val)\;
                        ReplaceInstWithInst(us, new)\;
                    } 
                }
            }
        }
        
        \textcolor{blue}{\tcc{Handle String Variables}}
        \If{$Instr$ is $AllocInstr$ $\land$ $Instr \in StringVars$}{
                ary $\longleftarrow$ CreateArray(Instr.str) \;
                gbl $\longleftarrow$ CreateGlobalVar(ary) \;
                \For{$us \in use(Instr)$}{
                    \If{$us$ is $StoreIntr$}{
                        new $\longleftarrow$ createStoreInstr(gbl) \;
                        ReplaceInstWithInst(us, new)\;
                    }
                }
        }
        }
      }
    % }
\end{algorithm}
\end{comment}

\begin{algorithm}[!htb]
\scriptsize
% \small
\caption{\lmcas Constant-Conversion}%\lmcas Constant Conversion
\label{alg:cc}
\DontPrintSemicolon
\KwIn{program P, Map <$V_s, C_s$>, NeckLocation=$L$}
\KwOut{$P_{cc}$}
    \SetKwProg{Def}{def}{:}{}
    $P_{cc} \leftarrow P$ \;
    
    \textcolor{blue}{\tcc{Configuration Logic CC}}
    ConstantConversion(PreNeck($P_{cc}$), Map) \;
    
    \textcolor{blue}{\tcc{Main Logic CC}}
    \For{$var \in Map.keys$}{
        identify aliases of $var$\; \label{alg:l:alias}
        \If{none of the aliases modify the address $var$ after $L$ }{\label{alg:l:alias-b}
            add all $var$'s aliases to $Map$\; \label{alg:l:alias-e}
        } \Else{
            remove $var$ and its value from $Map$ \;
        }
    }
    ConstantConversion(PostNeck($P_{cc}$), Map) \;
    
    \Def{ConstantConversion(ProgamPart, Map)}{
    %   \Repeat{$Instr == Loc$}{
       \For{$Instr \in ProgamPart$}{
        \If{$Instr$ is $LoadInstr$}{\label{alg:l:fndLoadInst}
            \textcolor{blue}{\tcc{Handle Global Variables}}
            \If{oprnd is Global Variable}{\label{alg:l:globals-b}
                $replaceInstrWithConst(Map[oprnd])$\;
            }\label{alg:l:globals-e}
            \textcolor{blue}{\tcc{Handle Base Variables}}
            \If{oprnd is a Base Variable}{\label{alg:l:base-b}
                $replaceInstrWithConst(Map[oprnd])$\;
            }\label{alg:l:base-e}
        }
        \textcolor{blue}{\tcc{Handle Pointer to Base Variables}}
         \If{$Instr$ is $StoreInstr$}{ \label{alg:l:PtrToBase-b}   
            \If{destination operand (destOprd) is a pointer to Base Variable}{ \label{alg:l:PtrBaseVars}
                new $\leftarrow$ createStoreInstr(Map[destOprd],destOprd)\;\label{alg:l:PtrToBase-replc1}
                ReplaceInstWithInst(Instr, new)\;\label{alg:l:PtrToBase-replc2}
            }
        }\label{alg:l:PtrToBase-e}
        
        \textcolor{blue}{\tcc{Handle Struct \& Pointer to struct Variables}}
        \If{$Instr$ is $GEPInstr$}{ \label{alg:l:strctPtrToStrct-b}
            \If{oprnd is a struct/pointer to struct}{ \label{alg:l:strctPtrToStrct-traceBack}
                \For{Find $StoreIntr$ uses $GEPInstr$}{\label{alg:l:strctPtrToStrct-findStor}
                    new $\leftarrow$ createStoreInstr(Map[oprnd],oprnd)\;
                    ReplaceInstWithInst($StoreIntr$, new)\;
                }\label{alg:l:strctPtrToStrct-e}
            }
        }
        
        \textcolor{blue}{\tcc{Handle String Variables}}
        \If{$Instr$ is $AllocInstr$ and $Instr$ String Variable}{ \label{alg:l:strgVar}
            ary $\leftarrow$ CreateArray(Map[$Instr$]) \;\label{alg:l:crtAry}
            gbl $\leftarrow$ CreateGlobalVar(ary) \;\label{alg:l:crtGbl}
            \For{Find $StoreIntr$ uses $AllocInstr$}{\label{alg:l:findstrStore}
                new $\leftarrow$ createStoreInstr(gbl, $AllocInstr$) \;
                ReplaceInstWithInst($StoreIntr$, new)\;
            }\label{alg:l:replaceStoreStr}
        }
    }
    % }
    }
\end{algorithm}

\begin{algorithm}[!htb]
\scriptsize
\caption{\lmcas Clean up}
\label{alg:cp}
\DontPrintSemicolon
\KwIn{$P_{cc}$, visitedFunc}
\KwOut{$P$\textprime}
    \SetKwProg{Def}{def}{:}{}
    % \Def{CleanUp($P_{cc}$)}{
    $P\textprime\leftarrow P_{cc}$ \;
       \textcolor{blue}{\tcc{Remove unused functions}}
       CG $\leftarrow$ constructCallGraph($P_{cc}$) \;
       \For{$func \in CG$}{
        \If{$func\notin visitedFunc~\land$ $func$ is not operand of other instructions}{%use(func) == 0
            % \If{$use(func) == 0$}{
                remove(func) \;
            % }
        }
      }
      \For{$func \in CG$}{
        \If{$func$ is not operand of other instructions}{%$use(func) == 0$
            removeNodeAndItsDescendant(func) \;
        }
      }
      \textcolor{blue}{\tcc{Remove unused Global Variables}}
      \For{$var \in getGlobalList(P_{cc})$}{
        \If{$var$ is not operand of other instructions}{%$use(var) == 0$
            remove(var) \;
        }
      }
      \textcolor{blue}{\tcc{Remove unused Stack Variables}}
      \For{$func \in CG$}{
        \For{$inst \in func$}{
            \If{$inst$ is $AllocInst$}{
                \If{$inst$ is not operand of other instructions}{ %$use(inst) == 0$
                    remove(inst) \;
                }\uElseIf{$inst$ is a destination operand of only one $storeInst$}{ %$use(inst) == 1$ $\land$ $use(inst)$ is $StoreInst$
                    remove($storeInst$) \;
                    remove($inst$) \;
                }
            }
        }
      }
    % }
\end{algorithm}

\subsection{Multi-Stage Simplification (MS)} \label{subsec:msp}
\Omit{\vr{It is surprising you do not mention any of the dead code elimination passes.
LLVM also has a standard sequence of passes based on optimization level. Some of
these passes may be repeated. An informed reader will expect that you either use
the standard sequence or have repetitions of passes to get better optimization.} \ma{ Good point. But I mentioned in the clan up step that LLVM has passes to remove unused code and explained our motivation about not to use the standard dead code elimination passes}}

\Omit{\vr{Apparently LTO can remove unused functions.\\
\url{https://stackoverflow.com/questions/6687630/how-to-remove-unused-c-c-symbols-with-gcc-and-ld}\\
\url{http://lists.llvm.org/pipermail/llvm-dev/2020-January/138660.html} \ma{I didn't come across LTO, I relied on this LLVM documentation to find standard LLVM passes. https://releases.llvm.org/6.0.0/docs/Passes.html}. There is a post (scored 19) on the link that you shared says the generated app was buggy}}
\Omit{\vr{Also, StoreInst not being removed is surprising at least. Maybe give more reason
why that would happen. Just looking very briefly around, it seems StoreInst
removal is supported in dead code elimination.\\
\url{https://github.com/llvm-mirror/llvm/blob/master/lib/Transforms/Scalar/DeadStoreElimination.cpp\#L782}
\ma{Good point. I mentioned how and why this can happen "variables that are initialized but ended up unused"}}}

After variables have been converted to constants, the next step is to perform \Omit{\twr{whole-program}}whole-program optimization to simplify the code and remove unnecessary code.\Omit{\vr{slightly reworded next sentence.}\ma{thanks}}
In this phase, we used existing LLVM passes as well as wrote our own pass to perform powerful simplifications at different levels of granularity in the programs.
In particular, \lmcas uses the standard LLVM pass for constant propagation to perform constant folding;
it then uses another standard LLVM pass to simplify the control-flow.
\Omit{\twr{Is the following pass the one you wrote?
There is a difference in nuance between "we apply an LLVM pass customized"---which implies that you modified an existing pass---versus "we wrote our own pass"---which means that the pass is your own.  Above you said "wrote our own pass", but the language used here does not match.}\ma{The MS phase uses 2 standard LLVM passes and 1 LLVM pass wrote by me, as mentioned at the beginning of this paragraph. I agree the description thereafter was vague. I fixed that}}
Finally, it applies \Omit{\twr{a custom LLVM pass}}our LLVM pass implemented to handle the removal of unnecessary code. 
\Omit{
\twr{I think it is a mistake to state "cheap optimization" as the chief criterion. \ma{I'll rewrite it} What is missing is : "The next step is to perform interprocedural constant folding, plus removal of useless and unreachable code." What I understood you to say was that there was no single LLVM pass that performs that work, so you designed your own using a collection of standard LLVM passes (most of which work intraprocedurally) together with passes of your own design\ma{yes, correct summary}.  Section 3.4 should tell that story.  I suspect it is not relevant to even mention "cheap optimization".}\ma{got your point, I modified the beginning of Section 3.4}}
%Our goal is to conduct a cheap optimization, but still leads to powerful simplification at different granularity levels in the debloated programs. %without incurring overhead.
% In this phase, we perform the simplifications by means of standard LLVM passes:
\begin{itemize}
    \item \textbf{Constant Propagation}.
    This optimization step folds variables that hold known values by invoking the standard LLVM constant-propagation pass.
    \Omit{\twr{Unnecessary: "by passing \texttt{constprop} as an argument of the LLVM command \texttt{opt}."  That is some minor detail of your implemenation.} \ma{ got it}}Constant folding allows instructions to be removed.
    It also opens up the opportunity for additional simplifications, such as
    ``Simplifying CFG'' below.
    \item \textbf{Simplifying the CFG}.
    \lmcas benefits from the folded constants in the previous step to make further simplifications to the control-flow graph.
    \lmcas leverages a standard LLVM pass, called \texttt{simplifycfg}, to obtain these simplifications.
    This pass determines whether the conditions of branch instructions are always true or always false:
    unreachable basic blocks are removed, and basic blocks with a single predecessor are merged.
    The simplifications in this pass are achieved at the basic-block level. 
    \item \textbf{Clean Up}.\Omit{\twr{I think you need to say more about what was lacking in LLVM.} \ma{ I'll do}} %there is no a dedicated LLVM pass that handles the removal in strategic way to minimize the analysis time. For example although the LLVM pass aggressive dead code elimination (ADCE) aggressively tries to eliminate code, but it does not remove unused functions. It assumes values are dead until proven otherwise, which requires iterating all instructions. The removal of global variables and unused functions can be achieved by another LLVM pass. Hence, there is a pressing need to optimize the simplification step to avoid exhaustive process of applying standard LLVM passes. The clean up step achieves this goal by applying a strategic way, which starts by removing unused functions then removing global and stack variables. 
    In the simplification pass, \lmcas removes useless code (i.e., no operation uses the result~\cite{cooper2011engineering}) and unreachable code, including dead stack and global variables and uncalled functions.
    Although LLVM provides passes to perform aggressive optimization, we wrote a targeted LLVM pass that gives us more control in prioritizing the cleaning up of unneeded code, as described in Algorithm~\ref{alg:cp}.
    
    \hspace*{1.5ex}
    The first priority is to remove unused functions.
    \Omit{
    \twr{Once again, start off by stating the goal.  What functions are you trying to remove?  To characterize them, two categories might be (i) called only from call-sites before the neck, but not called during SE, and (ii) never called from the set of functions transitively reachable from \texttt{main} (including indirect call-sites).} \ma{thanks for the pointers. I modified the description.}}
    The goal is to remove two categories of functions:
    (i) those that are called only from call-sites before the neck, but not called during symbolic execution (this step is performed in Algorithm~\ref{alg:cp} Lines 4-6), and (ii) those that are never called from the set of functions transitively reachable from \texttt{main} (including indirect call-sites), as described in Algorithm~\ref{alg:cp} at Lines 7-9.
    Function removal is performed after constructing the call graph at Line 3.\Omit{\ma{I added the following for discussing indirect call sites}} Algorithm~\ref{alg:cp} also checks the number of uses of a function at Lines $5$ and $8$ before removing the node to handle indirect call sites. This check prevents the removal of a function used via a function pointer.
    %We first construct the call graph and%check the usage of each node starting from the entry point (i.e., function \textit{main}).
    \Omit{\twr{What is the difference in information content between "not in ... visited" and "number of uses is zero".} \ma{ I'll clarify that}} 
    %iterate over it twice.
    %The first category of functions in the first iteration (Lines 4-6). Specifically, we remove nodes that are not in the list of visited functions and the number of uses is zero because the list of visited functions is a non-exhaustive list as the program is executed up to the neck. The second iteration loops over the updated call graph starting from the entry point (i.e., function \textit{main}) and removes the second category of functions nodes that have zero uses and their descendant nodes.
    
    \hspace*{1.5ex}
    The focus then shifts to simplifying the remaining functions.
    For removing global variables (Lines 10-12), we iterate over the list of global variables obtained through the LLVM API \texttt{getGlobalList} and remove unused variables.
    Finally, we remove stack variables (Lines 10-13), including initialized but unused variables by iterating over the remaining functions and erasing unused allocation instructions.
    (In general, standard LLVM simplifications do not remove a stack variable that is initialized but is not otherwise used because the function contains a store operation that uses the variable.
    Our clean-up pass removes an initialized-but-unused variable by deleting the store instruction, and then deleting the allocation instruction.)
    
\end{itemize}

\Omit{\twr{Wording changes OK?} \ma{Yes, thanks}}
This phase performs simplifications at both the function level and the instruction level. Consider again the motivating example to create a specialized version of the word-count program (cf., Listing~\ref{wc}) that only counts lines (cf., Listing~\ref{wc-cl}).
After performing the \Omit{\twr{constant-conversion}}constant-conversion phase, both the \texttt{count\_chars} and \texttt{count\_lines} fields of the struct pointed to by stack variable \texttt{flag} are replaced by the constant values $0$ and $1$, respectively (See Table~\ref{tab:vars}).
The simplification steps remove the tests at lines $18$ and $20$ because the values of the conditions are always true.
Because the values of the conditions in the tests at lines $17$ and $19$ are always false, control-flow simplification removes both the tests and the basic blocks in the true-branches.
Furthermore, the removal of these basic blocks removes all uses of the global variable \texttt{total\_chars}, and thus the cleanup step removes it as an unused variable. 

%The performed multistage simplifications satisfy our requirements to make the simplifications at various granularity levels.





==> background.tex <==
\section{Background} \label{sec:background}
In this section, we provide the necessary background on program analysis and software debloating that will be used in the remainder of the paper. 

\noindent\textbf{Symbolic execution~\cite{SymbolicExecution} and partial evaluation~\cite{partialEvaluation}:} are generalizations of standard interpretation of programs, but there are key differences between them. Specifically, symbolic execution permits interpretation of a program with symbolic values, while partial evaluation precomputes program expressions in terms of the known static input. Therefore, partial evaluation specializes a program with respect to a subset of its input, which is know as \emph{supplied inputs}. In effect, partial evaluation performs optimizations such as loop unrolling, constant propagation and folding, function in-lining, etc. to produce the residual program~\cite{WIPER}. Hence, in contrast to symbolic execution the result of a partial evaluator (i.e. program specializer) is not the value of output variables, but another program (know as residual program or specialized program). Both techniques have been employed together to accomplish various tasks (i.e. software verification~\cite{Interleaving}).

%\textbf{Partial Evaluation (PE)~\cite{partialEvaluation,slicing,tutorialPE}}: is an optimization and specialization technique that precomputes program expressions in terms of the known static input. Therefore, partial evaluation specializes a program with respect to a subset of its input, which is know as \emph{supplied inputs}. In effect, partial evaluation performs optimizations such as loop unrolling, constant propagation and folding, function in-lining, etc. to produce the residual program~\cite{WIPER}.

%I need to rephrase this paragraph, I took it from ARDiff (FSE)
%\textbf{Symbolic Execution~\cite{SymbolicExecution}}: a static program analysis technique that uses symbolic rather than concrete values to represent program inputs – is one popular approach for establishing functional equivalence. With symbolic execution, a program is represented by a first-order logic formula over symbolic variables, which captures each program execution path as a conjunction between path condition and path effect: the first is the formula constraining values that enable the executing of the path and the second describes values computed along the path. This representation is referred to as a program symbolic summary. Establishing functional equivalence between two versions of a program then translates into the problem of establishing equivalence between their summaries, usually using solvers for Boolean Satisfiability (SAT) or Satisfiability Modulo Theories (SMT)~\cite{smt}.

\rev{
\noindent\textbf{KLEE}
\noindent\textbf{LLVM}
}

\noindent\textbf{Stack Variables:} temporary variables created by each function. For instance, the variables \emph{count\_chars} and \emph{count\_lines} are stack variables. Every time a function declares a new variable, it is "pushed" onto the stack. Then every time a function exits, all of the variables pushed onto the stack by that function are deleted. Once a stack variable is freed, that region of memory becomes available for other stack variables. 

% \noindent\textbf{Data Types in C/C++:}




==> discussion.tex <==
\section{Discussion and Limitation} \label{sec:discussion}

\begin{comment}
\begin{table*}[!htb]
\centering
\begin{threeparttable}
\caption{\twr{You might squeeze this table into one column by abbreviating OCCAM, TRIMMER, etc. and shrinking with resizebox.}
Comparison summary with state of the art debloating techniques}
\begin{tabular}{|p{4.2cm}|p{2cm}|p{2.43cm}|p{2cm}|p{1.5cm}|}
\hline
Metric & OCCAM~\cite{OCCAM} & TRIMMER~\cite{TRIMMER} & CHISEL~\cite{Chisel} & \textbf{\lmcas}\\\hline
Average Analysis Time (sec) & 2.69 & 7.2 & 4167.64 & \textbf{2.5} \\\hline
Size Reduction Rate & $22\%$ & $21\%$ & $91\%$ & $\textbf{25\%}$ \\\hline
ROP gadgets Reduction & 21.5\% & 28.5\% & 66.2\% & \textbf{51.7\%} \\\hline
\# of Evaluated Apps & 3\tnote{1} & 13 & 10 & \textbf{23}\\\hline
Open Source & $\cmark$ & $\xmark$ & $\cmark$ & \textbf{$\cmark$}\\\hline
\end{tabular}
\label{table:comparison}
   \begin{tablenotes}
     \item[1] \small The number of evaluated apps in the paper is $3$, but the number of the apps in OCCAM GitHub repository is more
   \end{tablenotes}
  \end{threeparttable}
\end{table*}
\end{comment}

\lmcas's main goal is to facilitate the process of debloating applications using a lightweight approach while maintaining reliability and soundness. We developed \lmcas to satisfy the five debloating requirements introduced in~\cite{Chisel}. %These requirements aim to generate reliable specialized applications. Therefore, 
Table~\ref{table:comparison} presents a comparison with prior work. 
\lmcas outperforms partial-evaluation-based approaches (OCCAM and TRIMMER) for application specialization.
Although it was infeasible to compare with TRIMMER experimentally because neither TRIMMER nor the specialized programs that it produced were available, \lmcas achieves better reduction rates compared to the results reported for TRIMMER.
\lmcas reduces the size of the binary by $25\%$, on average (see Figure~\ref{fig:avgReduction}), while TRIMMER reduces the size by $21\%$~\cite{TRIMMER}.

\begin{table}[!htb]
\centering
\caption{\label{table:comparison}Comparison summary with state-of-the-art debloating techniques.}
% \resizebox{\columnwidth}{!}{%
\scalebox{0.7}{
\begin{threeparttable}
% \begin{tabular}{|p{3.8cm}|p{2cm}|p{2.43cm}|p{2cm}|p{1.5cm}|}
\begin{tabular}{|p{2.8cm}|p{1.9cm}|p{2.2cm}|p{1.8cm}|p{1.2cm}|}
\hline
Metric & OCCAM~\cite{OCCAM} & TRIMMER~\cite{TRIMMER} & CHISEL~\cite{Chisel} & \textbf{\lmcas}\\\hline
Average Analysis Time (sec) & 2.69 & 7.2 & 4167.64 & \textbf{2.5} \\\hline
Size Reduction Rate & $22\%$ & $21\%$ & $91\%$ & $\textbf{25\%}$ \\\hline
ROP gadgets Reduction & 21.5\% & 28.5\% & 66.2\% & \textbf{51.7\%} \\\hline
\# of Evaluated Apps & 3\tnote{1} & 13 & 10 & \textbf{23}\\\hline
Open Source & $\cmark$ & $\xmark$ & $\cmark$ & \textbf{$\cmark$}\\\hline
\end{tabular}
   \begin{tablenotes}
     \item[1] \small The number of evaluated apps in the paper is $3$; the number of apps in OCCAM's GitHub repository is greater.
   \end{tablenotes}
  \end{threeparttable}}
\end{table}


While reinforcement-learning approaches like CHISEL can achieve a high reduction rate, the majority of the debloated programs that CHISEL produces either crash or do not work properly in some other way.
CHISEL's analysis is conducted on top of the source code without including libraries.
In contrast, \lmcas performs its analysis over the LLVM IR using bitcode that includes the code for all libraries.
Furthermore, CHISEL suffers from overhead and usability issues because the developer potentially needs to create many test cases to cover even a single debloating scenario.
\Omit{\twr{The ideal here is to say what the threat to validity are, and what we did to mitigate the threats.}}
In the following, we outline threats to the validity of our approach along with the applied mitigations: 
\begin{itemize}
    \item \textbf{Incorrect neck identification}. Misidentifying the neck may
      lead to incorrect debloating. For example on of our requirements constrains the neck candidates by the property that the neck is executed only once.
      As a corollary, the neck cannot appear in a loop.
    \Omit{\twr{Restatement OK?  There used to be something about dominance, but it didn't make sense.} \ma{thank, Tom. the rewording clarifies the mitigation better now}}
    \Omit{\vr{I rewrote this. Feel free to discard if you don't like.}}
    \Omit{\vr{While correct, needs rewording. \#2 probably subsumes \#1. Also, the
    dominance is guaranteed only under a specific input assignment.} \ma{How about this? if still not satisfying. Can you please help to improve the wording.}}
    
    \hspace{1.5ex}
    \Omit{\twr{Moved here from Sect.~\ref{subsec:neck}, as it represents a threat to validity.}}
    There can be situations where the some approaches to neck identification discussed in  Sect.~\ref{subsec:neck} fails;
    in particular, the criterion of finding a dominator in the CFG may not be the right condition.
    For instance, suppose that the application is essentially the union of two separate applications $A_1$ and $A_2$ that share some common code $C$;
    suppose that they were combined by introducing a command-line parameter that causes a dispatch to one of two different places (corresponding to $A_1$ and $A_2$), at which point subsequent app-specific command-line processing is performed, and then $A_1$ or $A_2$ is run (and both ultimately call the common code $C$).
    Note that $C$ is not dominated by either the end of command-line processing for $A_1$ (say, $a_1$) or the end of command-line processing for $A_2$ ($a_2$).
    In this case, one would want the neck to be a cut-set: $\{ a_1, a_2 \}$.
    Although this situation is possible, in our somewhat limited experience to date, we have not encountered it.
    Moreover, it is essentially trivial to change from working with a single-point neck to working with a cut-set neck (i.e. in this case neck is a set of statements).
    
    %However, other strategies, including heuristic analysis techniques, could be applied to aid neck identification. For instance, the GNU CoreUtils programs use a particular idiom for parsing command-line parameters; in principle, a special-purpose algorithm could be designed for identifying the neck for programs that use that idiom.  
    
    \item \textbf{Precision of Constant Conversion}.
    \Omit{\vr{Feels verbose for PLDI. Maybe just say: LMCAS performs a
      conservative but sound conversion of variables into constants.}}\Omit{\twr{Wording of this part OK?}\ma{yes, thanks}}\lmcas relies on converting a subset of the variables into constants.
    If one of the variables could have been converted to a constant, but was not identified by \lmcas as being convertible (and therefore no occurrences of the variable are changed), no harm is done: that situation just means that some simplification opportunities may be missed.
    On the other hand, if some variable occurrences are converted to constants unsoundly, the debloated program may not work correctly.
    
    \hspace{1.5ex}
    We mitigate this issue by: (1) avoiding the conversion of some variables to constants (e.g., \texttt{argc}) because the symbolic-execution input is different than the one required by the specialized program: for instance, with \texttt{wc} the file name is not supplied during symbolic execution, while the file name is supplied to the debloated program; 
    (2) leveraging existing LLVM APIs (i.e., \texttt{getUser}) that track the uses of variables to capture the final constant values at the end of the symbolic execution.
    This approach overcomes situations where a pointer indirectly updates the value of a location, and ensures that the \Omit{\twr{OK?}\ma{Yes, thanks}} pre-neck constant-conversion step operates using updated and accurate constant values.
    (3) Limiting the constant-conversion after the neck to unmodified variables (where "unmodified" accounts for aliasing).
    \Omit{\vr{The content deserves better explanation. The only thing I understand
    from this right now is that you have a sound (but possibly conservative)
    alias analysis.} \ma{yes, that's true.}}
    
    \Omit{\twr{I don't understand the next sentence.} \ma{I restate what we did in the Main Logic Constant-Conversion. Basically, the variable won't be converted to constant until we check that none of the alias variables is modified}}
    %While the conversion after the neck is limited to the variables that have not be modified, but after affirming the alias variables are not modified as well. 
    \Omit{\twr{What are you trying to say in the next three sentences?  I read it as saying that \lmcas needs to perform dataflow analysis, but you did not implement dataflow analysis.  However, my understanding is that you used existing LLVM dataflow passes, as well as at least one of your own design. If that is the case, then what is the threat to validity?} \ma{I our approach partially managed to overcome some of the challenges. For example, we don't perform inter-procedural constant propagation.}}
    %However, this does not substitute the need to apply data-flow analysis, especially if the original program makes use of features like pointer arithmetic. Inter-procedural static analyses~\cite{PhASAR}, points-to analysis~\cite{svfPaper}, and interprocedural constant propagation~\cite{cooper2011engineering} are required to track memory locations that are referred to by pointer variables. Data-flow analysis tools such as SVF~\cite{svfPaper} and PhASAR~\cite{PhASAR} can be leveraged to identify precisely the variables that can be converted to constants.    

    \Omit{\item \textbf{Dynamically-linked Libraries}.
    Our KLEE-based symbolic-execution phase works on a complete program with all libraries already linked statically.
    \twr{I don't get the next sentence (which is awkwardly worded.  If I understand correctly, you are proposing a generalized tool in which the resulting debloated program will make use of dynamically linked libraries.  What is the threat to validity?}
    Therefore, we are planning to port the results of the KLEE analysis and apply them to an LLVM module that can be compiled to a dynamically-linked binary.}
\end{itemize}


==> evaluation.tex <==
% \vspace{-0.1cm}
\section{Evaluation}
\label{sec:evaluation}
%Tom suggested in 1/4/21 meeting to mention that KLEE doesn't handle optimized programs using O2.


This section presents our experimental evaluation of \lmcas.
We address the following research questions:
 
 \begin{itemize}
    \item \textbf{Efficiency:}
      What is the debloating performance of \lmcas with respect to \lmcas analysis time, and the amount that apps are reduced in size? (\ref{subsec:Efficiency})
    \item \textbf{Security:}
      Can \lmcas reduce the attack surface? (\ref{subsec:security})
    \item \textbf{Scalability:}
      How scalable is \lmcas in debloating large apps? (\ref{subsec:Scalability})
    \item \textbf{Robustness:} 
      How robust are the debloated programs produced by \lmcas? (\ref{subsec:robustness})
    % \item \rev{\textbf{RQ5:} What is the applicability of applying the neck and its properties to various programs?}
    % \item \rev{\textbf{RQ5:} What is the debloating capability of \lmcas?}
 \end{itemize}

\begin{comment}
\noindent\textit{\textbf{Implementation}}.\Omit{\twr{MISSING: we do not say how neck analysis was performed.} \ma{ manually, but based on the neck identification algorithm, by satisfying the requirement that  the neck should be executed only once and it dominates the main logic}}
In the current implementation of \lmcas, neck identification is performed manually, and all other steps are performed automatically.

The \lmcas user marks the neck location by adding a particular function call to the program being analyzed.
The user has the responsibility of identifying an appropriate neck location that satisfies the constraints defined in Section~\ref{subsec:neckSpec} (i.e., the neck should be executed only once, and should dominate the main logic).
For the $15$ GNU CoreUtils programs in \texttt{Benchmark\_1}, the total time to perform the manual analysis was $4$ hours.
After examining three programs, we noticed these programs use a particular idiom for parsing command-line parameters;
thereafter, neck identification for the rest of the programs was much quicker (around 10 minutes/program).

We modified KLEE 2.1~\cite{KLEE} to perform the Partial Interpretation phase and to stop and capture the set of affected variables and their corresponding values after the neck is reached. 
\rev{
In essence, KLEE is being used as an execution platform that supports “partial concrete states.” For LMCAS, none of the inputs are symbolic, but only part of the full input is supplied. In the case of word-count, the input is “wc -c”, with no file-name supplied. Only a single path to the neck is followed, at which point KLEE returns its state (which is a partial concrete state).
The second column in Tables \ref{tab:benchApps} \& \ref{tab:largeApps} describes the inputs supplied to KLEE for the different examples.
}
We also developed two LLVM passes using LLVM 6.0 to perform constant-conversion (CC) and the clean-up step of the MS phase.
\end{comment}


\noindent\textit{\textbf{Experimental Setup}}. Our evaluation relies on three datasets, as shown in Table~\ref{tab:dataset}.
\textit{Benchmark\_1} contains $15$ programs from GNU Coreutils v8.32 (see Table~\ref{tab:benchApps}).
\textit{Benchmark\_2} contains five programs obtained from ChiselBench (see Table~\ref{table:cve}).\footnote{https://github.com/aspire-project/chisel-bench}
\textit{Benchmark\_3} consists of three programs (see Table~\ref{tab:largeApps}). 
\rev{
The selection of programs in Benchmark_1 was motivated by their use in prior papers on software debloating. We used Benchmark_2 because it provides us a list of CVE vulnerabilities and corresponding apps; considering this dataset facilitates our evaluation of the removal of CVEs, and allows us to compare against the CVE-removal performance of Chisel. While Benchmark_1 shows the size-reduction performance and analysis time of our approach under simple settings.
%we exclude it from the CVE-removal evaluation in RQ4 because we do not have a list of CVEs for this dataset.
}
\begin{comment}
Our evaluation relies on three datasets, as shown in Table~\ref{tab:dataset}.
For RQ1, we used \textit{Benchmark\_1}, which contains $15$ programs from GNU Coreutils v8.32 (see Table~\ref{tab:benchApps}), to evaluate the reduction rate produced by \lmcas and the time for analysis.
\textit{Benchmark\_1} is also used in the security evaluation (RQ3).
\textit{Benchmark\_2} contains five programs (see Table~\ref{table:cve}) obtained from ChiselBench;\footnote{https://github.com/aspire-project/chisel-bench}
it is used in RQ1 and RQ3 to compare with the state of the art.
\textit{Benchmark\_2} is also used in the robustness experiment in RQ3. 
The programs in this dataset are listed in Table~\ref{table:cve}.
Finally, in RQ2, we used \textit{Benchmark\_3}, which consists of three programs (listed in Table~\ref{tab:largeApps}), to evaluate scalability. %Tcpdump and two apps from Binutils (more details in~\ref{subsec:rq2}).
\end{comment}

\Omit{\twr{MISSING: say what test suite you used to test debloated apps}\ma{I used one test case, and compared the output before and after debloating. If the output is the same, this indicates debloating is performed correctly}. 
\twr{Not sure what to say: that is not a very comprehensive approach.
At least you ran AFL on \textit{Benchmark\_3} for RQ2.
Could you still run AFL on the debloated programs in \textit{Benchmark\_1} and \textit{Benchmark\_2}?}\ma{I'll do that, but due to time limitation, I'll run AFL for 2-3 hrs/app}}

%The numbers that we report for the sizes of debloated binaries are obtained with the \texttt{size} command on the binaries created with \texttt{gcc -O2}.

All experiments were conducted on an Ubuntu $18.04$ machine with a 2.3GHz Quad-Core Intel i7 processor and 16GB RAM, except the fuzzing experiment (RQ2), for which we used an Ubuntu $18.04$ machine with a 3.8GHz Intel(R) Core(TM) i7-9700T CPU and 32GB RAM.

\begin{table}[!tb]
\centering
\caption{Benchmark sets used in the evaluation.}
% \vspace{-0.4cm}
\scalebox{0.9}{
\begin{tabular}{llcl}
\hline
Source & Label & \# of apps & Scope \\ \hline 
\thead{GNU Coreutils 8.32} & Benchmark\_1 & 15 & RQ1, 2, 4 \\ \hline
\thead{CHISEL Benchmark} & Benchmark\_2 & 5 & RQ1, 2, 4\\ \hline
\thead{Tcpdump \& GNU Binutils} & Benchmark\_3 & 3 & RQ3 \\ \hline
\end{tabular}
}
\label{tab:dataset}
\end{table}


\noindent\textit{\textbf{Compared tools and approaches}}. To evaluate the effectiveness of \lmcas, we compared with the following tools and approaches:
\begin{itemize}
\begin{comment}
    \item
    \textit{Manual debloating}. %Best-effort
     We developed a simple but systematic protocol to perform debloating manually, which we state as Algorithm~\ref{alg:manualAlg}. The goal of this manual approach is to create a baseline for the maximum level of reduction that can be achieved by an average developer.\Omit{\twr{Comments on Algorithm~\ref{alg:manualAlg}.
    The second removal loop is still not satisfactory.
    Unintelligible to the reader: lines 16, 17, 20, 21; you are assuming they understand certain operations that you never explain.\ma{at these lines, I just iterate the worklists varsToRemove and funcToRemove, and I remove each element from the list, so the while loop terminates.}
    Worse, I don't see how lines 15-18 do the correct thing: for a given function $f$ in funcToRemove, you need to check whether the program still has any call-sites that call $f$: if there are no call-sites, then you can remove $f$. But you have to keep iterating: you could have already considered $g$, which was kept because there was a call on $g$ in $f$.  Now you want to remove $g$ as well, and so on . . .\ma{If g calls f, but there is no call for g, then the definition of func g is removed, and in the next iteration the definition of f will be removed. I was using grep to search for the occurrences of functions/variables}
    Finally, there is the issue of indirect function calls. The simplest approach is that you need to know the set of functions whose address has been taken (say $f$, $g$, and $h$); then all indirect call-sites are considered as if they are calls on $f$, $g$, and $h$.  (If you have done points-to analysis, then the set can be narrowed to the set of functions that the points-to analysis tells you.)
    Line 16 is still completely mysterious---callSiteSet is never used.\ma{I fixed it}}\ma{A general note on the manual analysis, I didn't perform any program analysis, if a variable/function is accidentally removed, then the app won't be compiled successfully or the app will crash or generate wrong output. So I undo the last removal.So it's kind of try-error approach. The goal of this approach is constituting a baseline about the level of reduction that can be manually achieved by an average developer}}
    We first create work-lists of variables and functions that are candidates for removal (Lines~\ref{alg:l:varsToRemove}-\ref{alg:l:funcToRemove}). We then execute app $A$ under the control of GDB\footnote{https://www.gnu.org/software/gdb/}
    to identify the set of statements that are executed based on input $I$, as described in Algorithm~\ref{alg:manualAlg} at Line~\ref{alg:l:gdb}. The manual debloating is performed over two main loops. In the first loop at Lines~\ref{alg:l:loop1-b}-\ref{alg:l:loop1-e}, we iterate over all statements in the source code starting from the main function.  
    % at Line~\ref{alg:l:main}. 
    If the statement does not belong to the list of executed statements ($Executed$), then we remove the statement and record its variables in the list of candidate variables to be removed ($varsToRemove$), but if the statement is a callsite, the function name is recorded in $funcToRemove$.
    %One also identifies the list of variables \Omit{\twr{affected by the input?}\ma{yes}} affected by the input.
    %If the statement uses only irrelevant variables, then the statement is removed and the variables themselves are considered as candidates for removal.
    %If the statement is a call-site that will never be invoked, the statement is removed and the called function is added to a list of functions that are candidates for removal.
    In the second loop at Lines~\ref{alg:l:loop2-b}-\ref{alg:l:loop2-e}, one iterates over the lists of variables and functions that are candidates for removal: the goal is to identify functions never invoked and variables never used by performing text-based search to determine the occurrences of the variable/functions (Lines~\ref{alg:l:occrFunc} and~\ref{alg:l:occrVar}), so that they can be removed, if they appeared only once in the remained source code. Finally, we compile the app to verify that it builds correctly; otherwise, we put back the removed statements, including removed variables and functions in the iteration (Lines~\ref{alg:l:build-b}-\ref{alg:l:build-e}). 
    
    \hspace{1.5ex}
    %This method manually removes functions and variables irrelevant to the intended functionality.
    The resulting application is compiled and tested to see that it yields correct results.
    %We call this approach "best effort" because it 
    This approach does not require prior knowledge of the application or advanced experience in program analysis---and thus average developers should be able to apply it to obtain only desired functionality. 
    \end{comment}
    \item Baseline. We establish the baseline by compiling each app's LLVM bitcode at the -O2 level of optimization. This baseline approach was used in prior work~\cite{TRIMMER}.
    \item Manual debloating. We developed a simple but systematic protocol to perform debloating manually, which we state as Algorithm $2$ (in the supplementary materials~\cite{materials}). The goal of this manual approach is to create a baseline for the maximum level of reduction that can be achieved by an average developer.
    \item OCCAM~\cite{OCCAM}. The system most comparable to the approach used by \lmcas. However, OCCAM does not perform constant propagation, and thus omits a major component of partial evaluation. 
    %that can be facilitated through constant propagation.
    \item CHISEL~\cite{Chisel}. It requires the user to identify wanted and unwanted functionalities and uses reinforcement learning to perform the reduction process. 
    \item RAZOR~\cite{RAZOR}. similar to CHISEL, RAZOR relies on test cases to drive the debloating, but also incorporates heuristic analysis to improve soundness. 
    \item Nibbler~\cite{Nibbler2}. state-of-the-art tool for debloating binary code. It does not generate specialized apps, it rather focuses only on reducing the size of shared libraries. 
    \begin{comment}
    \rev{
    We avoided running Chisel on Benchmark\_1, not only because its analysis takes a long time, but also because it requires transforming the programs into a single meta-file, generating test cases, and writing a script according to a certain template to identify the required features. These steps are a time-consuming process.
    }
    \end{comment}
\end{itemize}

\begin{comment}
\begin{algorithm}[!htb]
\caption{Best-Effort Manual Debloating Protocol}
\label{alg:manualAlg}
\DontPrintSemicolon
%\SetKwInOut{Require}{Require}
\KwIn{App $A$, Input $I_s$}
\KwOut{App $A\textprime$ }
  $relevantVars \longleftarrow \emptyset$\;
  $varsToRemove \longleftarrow \emptyset$\;
  $funcToRemove \longleftarrow \emptyset$\;
  $notExecuted \longleftarrow$ the set of statements that will not be executed, given input I \;
    \SetKwProg{Def}{def}{:}{}
    \Def{Debloat($A, I_s$)}{
      $A\textprime \longleftarrow A$ \;
      \Repeat{no more stmt removal}{
        %   Go to the main function\;
          \For{$stmt \in A\textprime$}{
            \uIf{$stmt$ is  $callSite$ \&\& $notExecuted$}{
               $A\textprime \longleftarrow remove(stmt)$\;
               $funcToRemove \longleftarrow add(func)$\;
            }%\Else{
                \uIf{$stmt(vars) \in I$}{
                    % $relevantVars \longleftarrow add(var)$ \;
                    relevantVars $\longleftarrow$ relevantVars $\cup$ \{var\} \;
                    $var \longleftarrow initVal(var)$\;
                }\Else{
                    $varsToRemove \longleftarrow add(var)$ \;
                    $A\textprime \longleftarrow remove(stmt)$\;
                }
            % }
          }
      
      \While{$varsToRemove$ $\neq \emptyset$ $ \land $ $funcToRemove$ $\neq  \emptyset$}{
            \For{$func \in funcToRemove$}{
            $callSiteSet \longleftarrow remove(func)$\;
            \uIf{func is not called}{
                %$A\textprime \longleftarrow remove(func)$\; 
                Remove func from A\textprime \;
                % $varsRemoval \longleftarrow add(func(vars))$\;
            }
          }
          \For{$var \in varsToRemove$}{
            $varsToRemove \longleftarrow remove(var)$\;
            \uIf{$var$ not used}{
                % $A\textprime \longleftarrow remove(var)$\;
                Remove var from A\textprime \;
            }
          }
      }
      }
    }
\end{algorithm}
\end{comment}


\begin{comment}
\begin{algorithm}[!htb]
\caption{Manual Debloating Protocol} %Best-Effort 
\scriptsize
\label{alg:manualAlg}
\DontPrintSemicolon
\KwIn{App $A$, Input $I$}
\KwOut{App $A\textprime$ }
  $varsToRemove \leftarrow \emptyset$\;\label{alg:l:varsToRemove}
  $funcToRemove \leftarrow \emptyset$\;\label{alg:l:funcToRemove}
  $Executed \leftarrow$ the set of statements that GDB reports are executed, given input $I$ \; \label{alg:l:gdb}
    \SetKwProg{Def}{def}{:}{}
    %   \While{runGDB($A, I$)}{
    %     $notExecuted \longleftarrow notExecuted \cup \{\textit{stmt}\}$
    %   }
      $A\textprime \leftarrow A$ \;
      \Repeat{no more removals of statements}{
        %   start from main \; \label{alg:l:main}
          \For{$stmt \in A\textprime$}{ \label{alg:l:loop1-b}
            \uIf{$stmt \not\in Executed$}{ \label{alg:l:execLst}
               remove stmt from $A\textprime$ \;
               $varsToRemove \leftarrow varsToRemove \cup \{\textit{stmt(vars)}\}$ \;
               \uIf{$stmt$ is a call site}{
                    $funcToRemove \leftarrow funcToRemove \cup \{\textit{func}\}$ \; \label{alg:l:loop1-e}
               }
            }
      \While{$varsToRemove$ $\neq \emptyset$ $ \land $ $funcToRemove$ $\neq  \emptyset$}{ \label{alg:l:loop2-b}
            \For{$func \in funcToRemove$}{
            % $funcToRemove \leftarrow remove(func)$\;
            Remove $func$ from funcToRemove \;
            \uIf{no occurrence of $func$ exists}{\label{alg:l:occrFunc}
                %$A\textprime \longleftarrow remove(func)$\; 
                Remove func from A\textprime \;
            }
          }
          \For{$var \in varsToRemove$}{\label{alg:l:occrVar}
            % $varsToRemove \leftarrow remove(var)$\;
            Remove $var$ from varToRemove \;
            \uIf{no occurrence of $var$ exists}{
                Remove var from A\textprime \;\label{alg:l:loop2-e}
            }
          }
      }
      \uIf{$A\textprime$ does not build correctly}{\label{alg:l:build-b}
        put back $stmt$ \;
        undo $var$ and $func$ removal from A\textprime\; \label{alg:l:undo}
      }\label{alg:l:build-e}
      }
     }
\end{algorithm}
\end{comment}

\begin{comment}
\begin{figure*}[h!]
\centering
% \vspace{-0.3cm}
  \subfloat[Average reduction in size achieved through manual debloating, OCCAM, and \lmcas, using four different size metrics. (Higher numbers are better.)]{
	\begin{minipage}[b][0.33\width]{
	   0.3\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{images/AvgReductionPerApp.pdf}
	   %\vspace{-0.5cm}
	   \label{fig:avgReduction}
	\end{minipage}}
 \hfill 
%  \vspace{-0.3cm}
  \subfloat[Running times of \lmcas, CHISEL, and OCCAM based on \textit{Benchmark\_2} (ChiselBench).]{
	\begin{minipage}[b][1\width]{
	   0.3\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{images/OCCAM_CHISEL_LMCAS_V2.png}
	   %\vspace{-0.5cm}
	   \label{fig:analysisTimeComparison}
	\end{minipage}}
 \hfill	

  \subfloat[Reduction in the total number of gadget occurrences (SYS, ROP and JOP) between \lmcas and OCCAM for \textit{Benchmark\_1}.  (Higher numbers are better.)]{
	\begin{minipage}[b][1\width]{
	   0.3\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{images/rop.png}
	   %\vspace{-0.5cm}
	   \label{fig:rop}
	\end{minipage}}
% 	\vspace{-0.3cm}
	\caption{Evaluation results of \lmcas}
\end{figure*}
\end{comment}

% \vspace{-0.3cm}
\subsection{Efficiency} \label{subsec:Efficiency}
We conducted two experiments to evaluate the efficiency of \lmcas.
First, we measured the reduction rate that \lmcas achieves, and compared it with two state-of-the-art tools.
Second, we measured the time required for performing partial interpretation and code simplification. 

\begin{table}[!tb]
\centering
\small
\caption{Characteristics of the benchmarks in \textit{Benchmark\_1}.}
% \vspace{-0.4cm}
\scalebox{0.9}{
\begin{tabular}{|p{1.3cm}|p{1.55cm}|p{0.8cm}|p{0.65cm}|p{1.1cm}|p{1cm}|}
\hline
\multirow{2}{*}{App} & \multirow{2}{*}{\shortstack{Enabled\\ Arguments}} &  \multicolumn{4}{c|}{Original} \\\cline{3-6}
 &  & \shortstack{\# IR \\ Inst.} & \shortstack{\#\\ Func.}  & \shortstack{\# Basic\\ Blocks} & \shortstack{Binary \\ Size $^a$} \\ \hline
basename & \-\-suffix=.txt & 4,083 & 96 & 790 & 26,672 \\ \hline
basenc & base64 & 8,398 & 156 & 1,461 & 44,583 \\ \hline
comm & -12 & 5,403 & 110 & 972 & 32,714 \\ \hline
date & -R & 29,534 & 166 & 6,104 & 89,489 \\ \hline
du & -h & 5,0727 & 466 & 8,378 & 180,365 \\ \hline
echo & -E & 4,095 & 89 & 811 & 27,181 \\ \hline
fmt & -c & 5,732 & 115 & 1,095 & 79,676 \\ \hline
fold & -w30 & 4,623 & 100 & 893 & 29,669 \\ \hline
head & -n3 & 6,412 & 119 & 1,175 & 37,429 \\ \hline
id & -G & 5,939 & 125 & 1,172 & 36,985 \\ \hline
kill& -9 & 4,539 & 96 & 898 & 31,649 \\ \hline
realpath & -P & 8,092 & 155 & 1,419 & 41,946 \\ \hline
sort & -u & 25,574 & 329 & 3,821 & 116,119 \\ \hline
uniq & -d & 5,634 & 115 & 1,092 & 37,159 \\ \hline
wc & -l & 7,076 & 130 & 1,219 & 41,077 \\ \hline
\end{tabular}}
\label{tab:benchApps}
\footnotesize{$^a$Total binary size obtained via the GNU \texttt{size} utility.}
\end{table}

\noindent\textbf{Reduction Rate}.
We used \textit{Benchmark\_1} to compare the performance of \lmcas against manual debloating, baseline, Nibbler, and OCCAM.
%(a) manually reduced programs, and (b) ones produced by the LLVM-based partial-evaluation tool OCCAM~\cite{OCCAM}:
%Figure~\ref{fig:avgReduction} summarizes the comparison results. Our approach achieves a higher reduction rate than the reduction rate in comparison with OCCAM. Interestingly, \lmcas also outperforms the manual debloating approach. This capability is illustrated in~\cite{Chisel}. This fact is underpinned by the capability of the automated approach to precisely remove all unused functions and instructions.
% Figure~\ref{fig:avgReduction} shows the average reduction in the binary size, achieved by manual debloating baseline (-O2), Nibbler, OCCAM, and \lmcas.
% All size measures, except binary size, are taken from the LLVM Intermediate Representation (IR).
Figure~\ref{fig:avgReduction} shows the comparison results based on the reduction in the binary size that each tool achieved for each app in \textit{Benchmark\_1}. For computing the binary-size metric, we compiled all debloated apps with \texttt{gcc -O2}, and ran \texttt{size}.
We report the sum of the sizes of all sections in the binary file (text + data + bss) because this quantity reflects the outcome of our simplifications across all sections. \lmcas achieved significant higher reduction rate (i.e., around the double) in comparison with manual debloating, baseline, and Nibbler.
%The function-reduction rate achieved via \lmcas is significantly greater than what is obtained via manual debloating. 
This result is due to the fact that the clean-up step of \lmcas can remove nodes in the call-graph that correspond to functions in binary libraries that are not used. 
%In contrast, the manual debloating approach (Lines 17-22 in Algorithm~\ref{alg:manualAlg}) does not have access to the source code of the binary libraries used. 
%systematically removes all unused functions, which is harder to do when debloating a program manually.
Although the reduction rates of \lmcas and OCCAM are close (geometric mean binary size reduction is $25\%$ and $22\%$, respectively), some of the specialized programs generated by OCCAM are not reliable.
In particular, of the applications in Table~\ref{tab:benchApps}, five of the OCCAM-debloated applications ($33\%$)  crash or generate inaccurate results. In contrast, all of the \lmcas-debloated applications run correctly (i.e., \lmcas preserves apps' behaviour).

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1\columnwidth]{images/AvgReductionPerApp.pdf}
    % \vspace{-0.5cm}
    \caption{Binary size reduction achieved through manual debloating, baseline, Nibbler, OCCAM, and \lmcas. (Higher numbers are better.)}
    \label{fig:avgReduction}
\end{figure} 

\begin{comment}

\begin{algorithm}[!htb]
\caption{Best-Effort Manual Debloating Protocol}
\label{alg:manualAlg}
\DontPrintSemicolon
%\SetKwInOut{Require}{Require}
\KwIn{App A, Input I}
\KwOut{App A\textprime \Omit{\twr{The procedure never uses A\textprime} \ma{ because it's the final output of the procedure}} }
  %$relevantVars \longleftarrow \emptyset$\;
  $irrelevantVars \longleftarrow \emptyset$\;
  $callSiteSet \longleftarrow \emptyset$\;
  
    \SetKwProg{Def}{def}{:}{}
    \Def{Debloat($A, I$)}{
      Go to the main function\;
      $update(relevantVar)$\;
      $update(irrelevantVars)$\;
      \twr{A function is different than a call-site; which do you mean? \ma{ initially, the callSiteSet contains a list of all functions in the program}  Also, why is the next statement an assignment but the later update of callSites not an assignment}\;
      $update(callSiteSet) \longleftarrow functions(A)$\;
      %while loop
      \While{$irrelevantVars$ $!=\emptyset$ $\&$ $callSiteSet$ $!=\emptyset$}{
            \For{$func \in callSiteSet$}{
            $callSiteSet \longleftarrow remove(func)$\;
            \uIf{func is not called}{
                $A \longleftarrow remove(func)$\; 
                $update(callSites)$\;
                $update(irrelevantVars)$\;
            }
          }
          \For{$var \in irrelevantVars$}{
            $irrelevantVars \longleftarrow remove(var)$\;
            \uIf{$var$ not used}{
                $A \longleftarrow remove(var)$\;
            }\Else{
                $replace(var) \longleftarrow initital(var)$\;
                $A \longleftarrow remove(var)$\;
            }
          }
      }
      $A \longleftarrow remove(irrelevant IncludeStmts)$\; 
    }
\end{algorithm}

\end{comment}

%We also explored other related tools, such as CHISEL~\cite{Chisel}. We compared \lmcas with CHISEL using \textit{Benchmark\_2}. Although CHISEL can achieve a high average reduction rate in the number of statements (i.e., $32.4\%$~\cite{Chisel}) and significant average reduction rate in the binary size of the apps, we found that all the resulting applications either crash, run forever, or return incorrect/empty results. Among the programs in \textit{Benchmark\_2}, all but one of the OCCAM-debloated programs work correctly, and all of the \lmcas-debloated applications run correctly.

\noindent\textbf{Running Time.} 
We measured the analysis time of \lmcas for \textit{Benchmark\_1}. The average total analysis time is $3.65$ seconds;
the maximum total analysis time is $13.08$ seconds for analyzing \texttt{sort};
and the minimum total analysis time is $1.19$ seconds for analyzing \texttt{basename}.
Notably, the time for constant conversion and multi-stage simplification is low:
on average, the time for constant conversion and multi-stage simplification is $0.4$ seconds, while the average time for Partial Interpretation is $3.25$ seconds.  
\begin{comment}
We measured the running time of \lmcas. Figure~\ref{fig:analysisTime} shows the breakdown of running time, for \textit{Benchmark\_1}, between (i) symbolic execution, and (ii) Constant Conversion (CS) plus Multi-stage Simplification (MS).

The average total running time is $3.65$ seconds;
the maximum total running time is $13.08$ seconds for analyzing \texttt{sort};
and the lowest total analysis time is $1.19$ seconds for analyzing \texttt{basename}.
Notably, the time for Constant Conversion and Multi-stage Simplification is low:
on average, the time for constant conversion and multi-stage simplification is $0.4$ seconds, while the average time for Partial Interpretation is $3.25$ seconds.  

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1\columnwidth]{images/TimeAnalysis.png}
    % \vspace{-0.6cm}
    \caption{The time required for symbolic execution and the partial-evaluation steps (Constant Conversion and Multi-stage Simplifications) for \textit{Benchmark\_1}.
    \Omit{\twr{Please change the label on the y-axis to "Running Time", and change the
    key from "CC \& MS" to "Partial Evaluation" to be consistent with the caption. We need \underline{all} labeling and terminology to be consistent \underline{everywhere}.}}}
    \label{fig:analysisTime}
\end{figure} 
\end{comment}

We also compared the running time of \lmcas against those of CHISEL, RAZOR, and OCCAM on \textit{Benchmark\_2}.
The results are shown in Figure~\ref{fig:analysisTimeComparison}.
The running times for \lmcas, RAZOR, and OCCAM are significantly lower than the time for CHISEL.
These results show that our debloating approach is more efficient than previous ones.
\lmcas substantially outperforms CHISEL and slightly outperforms OCCAM and RAZOR because it carries out a relatively lightweight debloating approach.
As a result, \lmcas runs up to $1500$x, $3.9$x, and $1.2$x faster on average than CHISEL, RAZOR, and OCCAM, respectively.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1\columnwidth]{images/OCCAM_CHISEL_LMCAS_V3.pdf}
    % \vspace{-0.8cm}
    \caption{\Omit{\twr{The y-axis says "Analysis Time''.  Make it consistent with the text, which I changed to ``running time''.}} 
    Running times of \lmcas, CHISEL, RAZOR, and OCCAM based on \textit{Benchmark\_2} (ChiselBench).}
    \label{fig:analysisTimeComparison}
\end{figure} 

\subsection{Security} \label{subsec:security}

We evaluated the capabilities of \lmcas to reduce code-reuse attacks and to remove known vulnerabilities.
We evaluated these security aspects from two angles: (i) we attempt to reproduce (by executing the app) the vulnerability after debloating the apps to see if the vulnerabilities were eliminated;
(ii) we measured the reduction in the number of code-reuse attacks\Omit{attack surface} by counting the number of\Omit{return-oriented programming (ROP)} eliminated gadgets in compiled versions of the original and reduced programs using ROPGadget~\cite{ROPGadget}, an analysis tool for enumerating different types of gadgets in a binary.

\noindent\textbf{Vulnerability Removal}.
To test the ability to mitigate vulnerabilities, we used the five programs in \textit{Benchmark\_2}.
Table~\ref{table:cve} presents a comparison between \lmcas, RAZOR, OCCAM, and CHISEL.
\lmcas and OCCAM removed CVEs from 4 out of the 5 programs, but the debloated \textit{sort-8.16} using OCCAM was not behaving correctly at run-time. While CHISEL and RAZOR removed CVEs from 3 programs. 
%the debloated sort using OCCAM is having infintie loop so it was stuck
\lmcas could not remove the vulnerability in \textit{date-8.21} because the bug is located in the core functionality of this program.
When undesired functionality is too intertwined with the core functionality---e.g., multiple quantities are computed by the same loop---then \lmcas may not be able to remove some undesired functionality because---to the analysis phases of \lmcas---it does not appear to be useless code.
%This situation hinders the removal of the CVE because \lmcas makes use of a conservative approach by mainly focusing on the removal of useless code, without conducting any simplification beyond that. 
In such cases, \lmcas retains the desired functionality. %---that required to run the program on the supplied arguments---without removing the undesired functionality of the program.
In contrast, CHISEL tries to remove all undesired functionality.
% \vspace{-0.3cm}
\begin{table}[!tb]
\centering
\caption{Vulnerabilities after debloating by \lmcas and CHISEL. $\cmark$ means the CVE vulnerability is eliminated; \Omit{\twr{Rewording OK?}} $\xmark$ means that it was not removed.}
% \vspace{-0.4cm}
\scalebox{0.75}{
\begin{threeparttable}
\begin{tabular}{llcccc}
\hline
App & CVE ID & RAZOR & CHISEL & OCCAM & \lmcas \\ \hline \hline
chown-8.2 & CVE-2017-18018 & $\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
date-8.21 & CVE-2014-9471 & $\cmark$ & $\xmark$ & $\xmark$ & $\xmark$ \\ \hline
rm-8.4 & CVE-2015-1865 & $\xmark$ & $\xmark$ & $\xmark$ & $\cmark$ \\ \hline
sort-8.16 & CVE-2013-0221 & $\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
uniq-8.16 & CVE-2013-0222 & $\xmark$ & $\cmark$ & $\cmark$ & $\cmark$\\ \hline
\end{tabular}
 \begin{tablenotes}
     \item[1] \small \revUN{CHISEL and RAZOR CVE removal is obtained from the corresponding publication.
     \item[2] \small Although OCCAM removed the CVE in rm-8.4, but the debloated version gets stuck at run-time.}
   \end{tablenotes}
  \end{threeparttable}
}
\label{table:cve}
\end{table}
% \vspace{-0.2cm}
% chown: I tried the attack here, but the specalized chown doesn't support -L https://lists.gnu.org/archive/html/coreutils/2017-12/msg00045.html
% $\xmark$ & $\cmark$

%date: I tried to run this command and our specialized date doesn't run this command 
%./date.bc_cu --date=TZ=123345 however, there are other websites use another string i.e. --date=TZ="123"345" @1

%rm: I tried the steps described here to reproduce the error, but worked correctly with me https://bugzilla.redhat.com/show_bug.cgi?id=1211300

%sort: I tried long input as specified in the description and nothing happened. it worked correctly. I couldn't find any specific steps to reproduce the bug

\noindent\textbf{Gadget Elimination}.
Code-reuse attacks leverage existing code snippets in the executable, called gadgets, as the attack payload~\cite{CSET19}.
Those gadgets are often categorized---based on their last instruction---into Return-Oriented Programming (ROP), Jump-Oriented Programming (JOP), and syscall (SYS)~\cite{Piece-Wise,CARVE}.
%ROP is a popular exploitation method used by attackers to bypass common defense mechanisms by corrupting the return address of an executing function. Upon its return, control is diverted to a gadget of the attacker’s choice~\cite{codeReuse,ROP,Saffire,Gadgets}. A SYS gadget involves a system-call instruction followed by a return instruction that might enable the execution of a kernel interrupt (system call).
Code-reuse attacks can be mitigated using software diversification, which can be achieved through application specialization.
Software debloating is a specialization technique that can both reduce the number of exploitable gadgets and change the locations of gadgets, thus diversifying the binary. 

In this experiment, we used \textit{Benchmark\_1} and observed noticeable reductions in the total gadget count \Omit{\twr{What are SYS and JOP? Are you saying that you have two other figures like Figure~\ref{fig:rop} for two other kinds of gadgets?  If so, break that out into a separate paragraph (after this one), and report an aggregate number like the geometric means for the SYS and JOP measurements.  Have I explained the subtleties of computing geometric mean of percentages to you?  You cannot just compute the geometric means of the raw percentage numbers.} \ma{I apologies for the incorrect description, but Fig 6 reports the 3 types of gadgets SYS, JOP and ROP. I fixed that by making sure everything is consistent that we report total gadgets}}(occurrences of ROP, SYS, and JOP gadgets), as illustrated in Figure~\ref{fig:rop}.
\Omit{\twr{How is average computed?  Say which kind of average you are reporting: arithmetic mean or geometric mean.} \ma{Arithmetic}}The average reduction (arithmetic mean) in the total number of gadgets is $51.7\%$ and the maximum reduction is $72.1\%$ (for \texttt{date}), while OCCAM reduces the total number of gadgets by $21.5\%$, on average, with a maximum reduction of $80.3\%$ (for \texttt{echo}).
For one program, \texttt{sort}, OCCAM increases the total number gadgets by $6.2\%$.
%A system-call instruction followed by \emph{ret} \Omit{\twr{will -> can? the issues is "definitely enables" versis "might enable"} \ma{I think it's safe to say might enable}} might enable the execution of a kernel interrupt (system call), and is called a \emph{system-call gadget}.
%We measured the reduction in system-call gadgets for \textit{Dataset\_1}.
 With \lmcas, the number of SYS gadgets is reduced to $1$ for $14$ out of the $15$ applications.
\lmcas caused an increase in the number of SYS gadgets in one application (\texttt{sort}), but still produced an overall decrease when considering ROP and JOP. A similar increase is also observed with TRIMMER in three applications~\cite{TRIMMER}.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{images/rop.png}
    % \vspace{-0.8cm}
    \caption{Reduction in the total number of gadget occurrences (SYS, ROP, and JOP) between \lmcas and OCCAM for \textit{Benchmark\_1}. (Higher numbers are better.)}
    \label{fig:rop}
\end{figure}

\subsection{Scalability} \label{subsec:Scalability}
We evaluated the capability of \lmcas to handle \textit{large-scale programs} that maintain complex input formats, such as object files, binaries, and network packets.

%\noindent\textbf{Large-Scale Programs}.\Omit{\twr{You already introduce the name \textit{Dataset\_3}, but nowhere in this paragraph do you refer to \textit{Dataset\_3}. The reader could think that you are introducing yet another dataset that you didn't tell him about.} ~\ma{I missed this}} 
We used \textit{Benchmark\_3} in this experiment. The programs considered in \textit{Benchmark\_3} have been used in prior work to evaluate scalability~\cite{OCCAM,SymCC}, including the scalability of KLEE~\cite{moklee}.
Accordingly, we use the following applications\footnote{
  Because deciding which lines of code belong to an individual application is difficult, lines of code (LOC) are for the whole application suites from which our benchmarks are taken.
  We used \texttt{scc} (https://github.com/boyter/scc) to report LOC.
}
to show the scalability of \lmcas: 
\begin{itemize}
    \item \texttt{tcpdump}~\cite{tcpdump} (version 4.10.0; 77.5k LOC) analyzes network packets.
    We link against %git #f030261 of 
    its accompanying libpcap library (version 1.10.0; 44.6k LOC).
    \item \texttt{readelf} and \texttt{objdump} from GNU Binutils~\cite{Binutils} (version 2.33; 78.3k LOC and 964.4k of library code\footnote{
      We only consider lines in the binutils folder and the following dependencies: libbfd, libctf, libiberty, and libopcodes.
      }).
      \texttt{readelf} displays information about ELF files, while \texttt{objdump} displays information about object files.
    %\item GNU objdump from GNU Binutils~\cite{Binutils} (version 2.33; 78.3k LOC and 964.4k of library code) displays information about object files.
\end{itemize}

We debloated these programs using different inputs to illustrate the capability of \lmcas to handle and debloat programs based on single and multiple inputs.
For example, we debloated \texttt{readelf} based on one argument \texttt{(-S)} and nine arguments \texttt{(-h -l -S -s -r -d -V -A -I)}. Table~\ref{tab:largeApps} breaks down the analysis time in terms of Partial Interpretation (third column) and the combination of Constant Conversion and Multistage Simplification (fourth column).
For these programs, the time for symbolic execution is lower than that for the LLVM-based simplifications.
This situation is expected because these programs contain a large number of functions, so a longer time is needed for the LLVM simplifications steps.
The inclusion of third-party libraries diminishes the reduction rate in the binary size, which is clearly illustrated in the achieved reduction rate for \texttt{tcpdump}. 

\begin{table}[!tb]
\centering
\caption{Scalability analysis of large applications, based on various inputs.
\Omit{\twr{This table is now inconsistent with Figure \ref{fig:analysisTimeComparison}: one refers to CC \& MS; the other refers to "partial-evaluation steps".  I prefer CC \& MS because it is more specific.} \ma{I fixed that, everything now is based on CC \& MS}} 
}
% \vspace{-0.4cm}
\small
\scalebox{0.9}{
\begin{tabular}{|p{1.2cm}|p{1.8cm}|p{0.8cm}|p{1.2cm}|p{1.9cm}|}
\hline
               App & Inputs & PI (sec) & CC \& MS (sec)& Binary Size\newline Reduction Rate\\ \hline
\multirow{2}{*}{tcpdump} & -i ens160 & 48.1 & 173.1 & 2\%\\ \cline{2-5}
                  & -i ens160 -c 5 & 48.2 & 201.7 &2\% \\ \hline
\multirow{2}{*}{readelf} & -S & 10.6 & 41.7 & 4.8\%\\ \cline{2-5}
                  & -h -l -S -s -r -d -V -A -I & 20.15 & 72.4 & 4.71\%\\ \hline
                 \multirow{2}{*}{objdump} & -x & 40.84 & 246.17 & 5.65\%\\ \cline{2-5}
                 & -h -f -p & 48.07 & 320.11 & 5.71\%\\ \hline
                 
\end{tabular}
}
\label{tab:largeApps}
\end{table}

\subsection{Robustness} \label{subsec:robustness}
We assessed the robustness of the debloated programs using fuzzing.
The aim was to test whether a debloated app functioned correctly and did not crash.
%we compiled all debloated apps (whether generated via \lmcas or another method~\ma{I'm currently running AFL on Dataset\_1 apps generated by LMCAS. If I have more time, I'll do it for the manually debloated apps}) with \texttt{gcc -O2} and ran it on the fuzzing tool AFL for 2 hrs/program.

We used AFL (version 2.56b), a state-of-the-art fuzzing tool~\cite{afl}, to perform this experiment.
AFL has been used to improve coverage~\cite{SymCC} and to verify robustness~\cite{Chisel}.
Because our analysis is performed on LLVM bitcode, we could not use AFL to instrument the source code (i.e., gray-box mode);
instead, we used AFL's black-box mode, which requires using the QEMU emulator (https://www.qemu.org/).
We compiled debloated programs with \texttt{gcc -O2} to generate the binary file for each program. 
Because black-box mode is 2-5x slower than gray-box mode, we ran AFL on the debloated programs created from \textit{Benchmark\_1} for 2 hours/program;
however, we ran AFL on the debloated programs created from \textit{Benchmark\_2} for six days.
AFL did not bring out any failures or crashes of the debloated programs in either dataset.
This experiment provides additional confidence in the correctness of the debloated programs created using \lmcas.


\begin{comment}
% \vspace{-0.3cm}
\rev{
\subsection{RQ5 (Debloating Capabilities)}
Table~\ref{tab:benchApps} presents \lmcas debloating settings for a subset of benchmark apps from Benchmark\_1 based on certain arguments (the second column) to conduct performance evaluation. However, \lmcas offers debloating based on various combination of input arguments and is not limited to the enabled arguments in the second column in Table~\ref{tab:benchApps}. Therefore, this section shows \lmcas's capability to perform debloating based on various input arguments for a subset apps from Benchmark\_1. For example, in  Table~\ref{table:capability}, \lmcas supports different arguments and/or combination of arguments to specialize apps according to the required functionalities. The last three columns provide the reduction rate w.r.t number of functions, binary size, and total gadgets in the generated specialized programs. We also ran AFL on the debloated programs and it did not report any failures or crashes.
}

\begin{table}[!htb]
\centering
\caption{\rev{Debloating subset apps from Benchmark\_1 based on various input arguments}}
\small
\scalebox{0.89}{
\begin{tabular}{|p{0.5cm}|p{1.45cm}|p{2.4cm}|p{1.4cm}|p{0.8cm}|p{0.95cm}|}
\hline
\multirow{2}{*}{App}  & \multirow{2}{*}{\shortstack{Enabled\\ Arguments}} & \multirow{2}{*}{\shortstack{Required\\ Functionality}}                     & \multicolumn{3}{l|}{Reduction After Debloating} \\\cline{4-6} 
                      &  &  & \#Functions & \shortstack{Binary \\ Size} & \shortstack{Total\\ Gadgets}   \\ \hline
\multirow{2}{*}{du}   & -b  & shows number of bytes & 23\% & 15\%  & 46\% \\ \cline{2-6} 
                      & -b --time                        & shows the time of the last modification and number of bytes & 22\%  & 14\% & 45\% \\ \hline
\multirow{3}{*}{sort} & -c                              & check if the file given is already sorted or not & 34\%          & 28\%         & 54\%                     \\ \cline{2-6} 
                      & -n & sort a file numerically & 31\%  & 25\%         & 51\% \\ \cline{2-6} 
                      & -un                             & sort a file numerically and remove duplicate     & 31\%          & 25\%         & 51\%                     \\ \hline
\multirow{4}{*}{wc} & -c & character count & 42\% & 21\% & 41\% \\ \cline{2-6} 
                      & -w & word count & 42\% & 21\% & 41\% \\\cline{2-6} 
                      & -lc & line and character count & 43\% & 22\% & 42\% \\ \cline{2-6} 
                      & -wc & word and character count & 42\% & 21\% & 42\% \\\hline
\end{tabular}}
\label{table:capability}
\end{table}
\end{comment}



